Score-Based Generative Modeling through Stochastic Differential Equations

Creating noise from data is easy; creating data from noise is generative modeling. We present a stochastic differential equation (SDE) that smoothly transforms a complex data distribution to a known prior distribution by slowly injecting noise, and a corresponding reverse-time SDE that transforms the prior distribution back into the data distribution by slowly removing the noise. Crucially, the reverse-time SDE depends only on the time-dependent gradient field (\aka, score) of the perturbed data distribution. By leveraging advances in score-based generative modeling, we can accurately estimate these scores with neural networks, and use numerical SDE solvers to generate samples. We show that this framework encapsulates previous approaches in score-based generative modeling and diffusion probabilistic modeling, allowing for new sampling procedures and new modeling capabilities. In particular, we introduce a predictor-corrector framework to correct errors in the evolution of the discretized reverse-time SDE. We also derive an equivalent neural ODE that samples from the same distribution as the SDE, but additionally enables exact likelihood computation, and improved sampling efficiency. In addition, we provide a new way to solve inverse problems with score-based models, as demonstrated with experiments on class-conditional generation, image inpainting, and colorization. Combined with multiple architectural improvements, we achieve record-breaking performance for unconditional image generation on CIFAR-10 with an Inception score of 9.89 and FID of 2.20, a competitive likelihood of 2.99 bits/dim, and demonstrate high fidelity generation of 1024 x 1024 images for the first time from a score-based generative model.

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method.tex <==
\section{Score-based generative modeling with SDEs}
Perturbing data with multiple noise scales is at the crux of the success of previous methods. We propose to generalize this idea further to an infinite number of noise scales, such that perturbed data distributions evolve according to an It\^{o} process as the noise intensifies. %

Note that when using a total of $N$ noise scales, each perturbation kernel $p_{\sigma_i}(\bfx \mid \bfx_0)$ in \cref{sec:ncsn} corresponds to the marginal distribution of $\bfx_i$ in the following Markov chain:
\begin{align}
\bfx_i = \bfx_{i-1} + \sqrt{\sigma_{i}^2 - \sigma_{i-1}^2} \bfz_i, \quad i=1,\cdots,N \label{eqn:ncsn},
\end{align}
where $\bfz_i \sim \mcal{N}(\bfzero, \bfI)$, and we have introduced $\sigma_0 = 0$ to simplify the equation. Let $r \triangleq (\nicefrac{\sm}{\sM})^2$. Because $\{\sigma_i\}_{i=1}^N$ is a geometric sequence, we have $\sigma_i = \sm r^{\frac{i-1}{2(N-1)}}$. In the limit of $N \to \infty$, the Markov chain $\{\bfx_i\}_{i=1}^N$ becomes a continuous process $\bfx(t)$, where we use a continuous time variable $t \in [0, 1]$ for indexing, rather than an integer $i \in \{1, 2, \cdots, N\}$. Let $\Delta t = \frac{1}{N-1}$, and $\bfx(\frac{i-1}{N-1}) = \bfx_i$. As $\Delta t \to 0$, \cref{eqn:ncsn} can be written as the following for $t \in \{\frac{1}{N-1}, \frac{2}{N-1}, \cdots, 1\}$ via Taylor expansion:
\begin{align*}
    \bfx(t) = \bfx(t-\Delta t) + \sm \sqrt{r^t - r^{t-\Delta t}}\bfz_i \approx \bfx(t-\Delta t) + \sm \sqrt{(r^{t-\Delta t}\ln r) \Delta t}~\bfz(t),
\end{align*}
and in the limit of $\Delta t = 0$, it converges to the following SDE for $t \in [0,1]$:
\begin{align}
\ud \bfx = \sm \bigg( \frac{\sM}{\sm} \bigg)^t \sqrt{2 \log \frac{\sM}{\sm}}\ud \bfw, \label{eqn:ncsn_sde}
\end{align}
where $\bfw$ is the standard Wiener process. Likewise for perturbation kernels $\{p_{\alpha_i}(\bfx \mid \bfx_0)\}_{i=1}^N$ in \cref{sec:ddpm}, the discrete Markov chain is
\begin{align}
    \bfx_i = \sqrt{1-\beta_{i}} \bfx_{i-1} + \sqrt{\beta_{i}} \bfz_i, \quad i=1,\cdots,N. \label{eqn:ddpm}
\end{align}
and the corresponding SDE can be obtained through a similar analysis (see Appendix):
\begin{align}
\ud \bfx = -\frac{1}{2}(\bbetam + t(\bbetaM - \bbetam)) \bfx(t) \ud t + \sqrt{\bbetam + t(\bbetaM - \bbetam)} \ud \bfw, \label{eqn:ddpm_sde}
\end{align}
where $\bbetam = (N-1) \betam$ and $\bbetaM = (N-1) \betaM$.

So far, we have demonstrated that the noise perturbations used in \citet{song2019generative} and \citet{ho2020denoising} both correspond to discretizations of SDEs. The SDE of \cref{eqn:ddpm_sde} yields a process with constant variance, as long as $p(\bfx_0)$ has variance one (proof in Appendix). In contrast, the SDE of \cref{eqn:ncsn_sde} always gives a process with exploding variance. Due to this difference, we hereafter refer to \cref{eqn:ncsn_sde} the variance exploding (VE) SDE, and \cref{eqn:ddpm_sde} the variance preserving (VP) SDE.

In general, we can consider noise peturbations that evolve according to any SDE:
\begin{align}
    \ud \bfx = \bff(\bfx(t), t) \ud t + \mbf{G}(\bfx(t), t) \ud \bfw. \label{eqn:forward_sde}
\end{align}
Here $\bff(\cdot, t): \mbb{R}^d \to \mbb{R}^d$ is a vector-valued function called the \emph{drift} coefficient, $\mbf{G}(\cdot, t): \mbb{R}^d \to \mbb{R}^{d\times d}$ is a matrix-valued function known as the \emph{dispersion} coefficient. %
In this work we follow the It\^{o} interpretation of SDEs. Under some regularity conditions~\citep{oksendal2003stochastic}, the solution to an SDE is an It\^{o} diffusion process $\bfx(t)$. We denote by $p_t(\bfx)$ the (marginal) probability density of $\bfx(t)$, and use $p_{st}(\bfx(t) \mid \bfx(s))$ to denote the transition kernel from time $s$ to $t$.%

We can use a continuous diffusion process to gradually diffuse an unknown distribution $p_0(\bfx_0)$, for which we have a dataset of \iid samples, to a known prior distribution $p_T(\bfx_T)$, for which we have a tractable form and can easily generate samples. 



By starting from $p_T(\bfx_T)$ and reversing the diffusion process, we can obtain $p_0(\bfx_0)$. This reverse process should yield the same trajectory of marginal probability densities $\{p_t(\bfx)\}_{t=0}^T$ as the forward SDE (\cref{eqn:forward_sde}), except that the evolution of $p_t(\bfx)$ is in the opposite time direction. A remarkable result from~\citet{Anderson1982-ny} states that the reverse of a diffusion process is also a diffusion process, running backwards in time. Moreover, the reverse diffusion process can be derived from the forward process, once the score of each marginal distribution, $\nabla_\bfx \log p_t(\bfx^t)$, is known for all $t$.
\begin{theorem}[\citet{Anderson1982-ny}, informal]\label{thm:reverse_sde}
The reverse process to \cref{eqn:forward_sde} is given by
\begin{align}
    \resizebox{0.935\textwidth}{!}{$\displaystyle\ud \bfx_t = \{\bff(\bfx_t, t) - \nabla \cdot [\bfG(\bfx_t, t) \bfG(\bfx_t,t)\tran] - \bfG(\bfx_t,t)\bfG(\bfx_t,t)\tran  \nabla_\bfx  \log p_t(\bfx_t)\} \ud t + \mbf{G}(\bfx_t, t) \ud \bar{\bfw}_t$},\label{eqn:backward_sde}
\end{align}
where $\{\bar{\bfw}_t\}_{t=T}^0$ is a standard Wiener process when time flows backwards from $T$ to $0$.\footnote{See Appendix for a rigorous statement.}
\end{theorem}
Throughout the paper we define $\nabla\cdot \mbf{F}(\bfx) := (\nabla \cdot \bff^1(\bfx), \nabla\cdot \bff^2(\bfx), \cdots, \nabla\cdot \bff^d(\bfx))\tran$ for a matrix-valued function $\mbf{F}(\bfx) := (\bff^1(\bfx), \bff^2(\bfx), \cdots, \bff^d(\bfx))\tran$. \cref{thm:reverse_sde} implies that the reverse diffusion is completely determined by the drift and dispersion coefficients of the forward process, as well as the \textbf{score} of its marginal probability density at each time step. Using \cref{thm:reverse_sde}, we can easily reverse \cref{eqn:forward_sde} to get samples from $p_0(\bfx_0)$, by simulating the trajectories of \cref{eqn:backward_sde}. The sampling procedure only requires 1) \textbf{score estimation} to obtain $\nabla_\bfx \log p_t(\bfx)$ of the forward SDE (\cref{eqn:forward_sde}), and 2) a \textbf{numerical SDE solver} to integrate the reverse-time SDE (\cref{eqn:backward_sde}).

\section{Estimating scores of the SDE}
The score of a distribution can be estimated by training a score-based model on samples with score matching~\citep{hyvarinen2005estimation, song2019sliced, song2019generative}. To estimate $\nabla_\bfx \log p_t(\bfx)$ with this approach, we shall choose a forward SDE (\cref{eqn:forward_sde}) whose perturbation kernel $p_{0t}(\bfx_t \mid \bfx_0)$ is solvable, so that we can easily generate training data from $p_t(\bfx)$ given data samples of $p_0(\bfx)$. One such example is linear SDEs.
\begin{proposition}[\citet{sarkka2019applied}, exact solution to linear SDEs]\label{prop:linear}
When the drift and dispersion coefficients in \cref{eqn:forward_sde} possess the form $\bff(\bfx_t, t) = \bfF(t)\bfx_t + \bfu(t)$ and $\bfG(\bfx_t, t) = \bfL(t)$, the transition kernel is $p_{0t}(\bfx_t \mid \bfx_0) = \mcal{N}(\bfx_t \mid \bfm(t), \bfsigma(t))$, where $\bfm(t)$ and $\bfsigma(t)$ are obtained by solving the following linear ODEs:
\begin{gather*}
\frac{\ud \bfm(t)}{\ud t} = \bfF(t)\bfm(t) + \bfu(t), \quad \bfm(0) = \bfx_0,\\
\frac{\ud \bfsigma(t)}{\ud t} = \bfF(t)\bfsigma(t) + \bfsigma(t)\bfF(t) + \bfL(t) \bfL(t)\tran, \quad \bfsigma(0) = \bfzero.
\end{gather*}
\end{proposition}
Typically we only have a dataset for $p_0(\bfx_0)$, but when an SDE is linear, we can employ the perturbation kernel provided by \cref{prop:linear} to directly obtain training data from $p_t(\bfx_t)$. Specifically, we first randomly select a data point $\bfx_0 \sim p_0(\bfx_0)$, and then draw $\bfx_t$ from the perturbation kernel $p_{0t}(\bfx_t \mid \bfx_0)$. Based on samples from $p_t(\bfx_t)$, we can use the following (infinite) mixture of score matching objectives to train a time-dependent score-based model $\bfs_\bftheta(\bfx, t)$ parameterized by $\bftheta$:
\begin{align}
    \min_\bftheta \mbb{E}_{\bfx_0 \sim p_0(\bfx_0)}\mbb{E}_{t\sim \mcal{U}(0, T)} \mbb{E}_{\bfx_t \sim p_{0t}(\bfx \mid \bfx_0)}[\lambda(t) \mcal{L}_{\text{SM}}(\bfs_\bftheta(\bfx_t, t), \bfx_0, \bfx_t)], \label{eqn:training}
\end{align}
where $\lambda: [0, T] \to \mbb{R}_{>0}$ is a positive weighting function, %
$\mcal{U}(0, T)$ denotes a uniform distribution over $[0, T]$, and $\mcal{L}_{\text{SM}}$ is a score matching loss function. With sufficient data, model capacity, and optimization accuracy, score matching ensures that the optimal solution to \cref{eqn:training}, denoted by $\bfs_{\bftheta^\ast}(\bfx, t)$, equals $\nabla_\bfx \log p_t(\bfx)$ for almost all $\bfx$ and $t$. Typical examples of $\mcal{L}_{\text{SM}}$ include denoising score matching (DSM,~\citet{vincent2011connection}), which can be written as 
\begin{align}
    \mathcal{L}_{\text{SM}} := \norm{\bfs_\bftheta(\bfx_t, t) - \nabla_{\bfx_t}\log p_{0t}(\bfx_t \mid \bfx_0)}_2^2. \label{eqn:dsm}
\end{align}
Other alternatives for $\mcal{L}_{\text{SM}}$ include sliced score matching~\citep{song2019sliced} and finite-difference score matching~\citep{pang2020efficient}.

\begin{figure}
    \centering
    \includegraphics[width=0.333\linewidth]{figures/NCSN_var.pdf}%
    \includegraphics[width=0.32\linewidth]{figures/ddpm_mean.pdf}%
    \includegraphics[width=0.32\linewidth]{figures/ddpm_var.pdf}
    \caption{Comparison of discrete-time perturbation kernels vs. continuous ones. \textbf{Left} compares the variance of perturbation kernels at different time steps on NCSN; \textbf{middle} compares the mean coefficients (the ratio of the mean to $\bfxd$) of perturbation kernels on DDPM; and \textbf{right} compares the variance of perturbation kernels on DDPM. }
    \label{fig:discretization}
\end{figure}

The training objectives of NCSN and DDPM can be unified as discretized approximations to \cref{eqn:training} when $\mcal{L}_{\text{SM}}$ is denoising score matching (\cref{eqn:dsm}). Using \cref{prop:linear}, we can analytically compute the perturbation kernels induced by the SDE of NCSN and DDPM. For NCSN, we have
\begin{align}
    p(\bfx_t \mid \bfxd) = \mcal{N}\bigg(\bfx_t; \bfxd, \sm^2 \bigg(\frac{\sM}{\sm} \bigg)^{2t}\bfI_d\bigg), \label{eqn:ncsn_sde_perturb}
\end{align}
while for DDPM,
\begin{align}
    p(\bfx_t \mid \bfxd) = \mcal{N}\bigg(\bfx_t ; e^{-\frac{1}{2}\bbetam t - \frac{1}{4}t^2 (\bbetaM-\bbetam)}\bfxd , \bfI_d - \beta_0 e^{\frac{1}{2}t(t-2)\bbetam-\frac{1}{2}t^2\bbetaM}\bfI_d\bigg).\label{eqn:ddpm_sde_perturb}
\end{align}
The original perturbation kernels $q_{\sigma_i}(\bfx \mid \bfxd)$ and $q_{\beta_i}(\bfx \mid \bfxd)$ for NCSN/DDPM are discretizations of \cref{eqn:ncsn_sde_perturb,eqn:ddpm_sde_perturb} at time steps $\{0, \nicefrac{1}{N-1}, \cdots, \nicefrac{N-2}{N-1}, 1\}$. 
\cref{fig:discretization} shows the near perfect agreement of discrete-time and continuous-time kernels when the number of noise scales $N$ is large. 

Our training method generalizes the original ones in NCSN/DDPM to an infinite number of noise scales, allowing flexible discretization and variable number of noise scales for sampling.





\section{Solving the reverse SDE}
After training a time-dependent score-based model, we can use it to construct the reverse SDE and then solve it to generate samples from $p_0(\bfx_0)$. Crucially, the additional knowledge of scores enables special numerical methods not applicable to general SDEs. These new methods not only provide better sample quality and efficiency, but also allow for exact likelihood computation, flexible manipulation of latent representations, and uniquely identifiable encoding/compression.

\subsection{General numerical solvers}
Numerical solvers provide approximate samples of trajectories from SDEs. Many general methods exist for the numerical integration of SDEs, based on different discretization and approximation strategies. Examples include Euler-Maruyama, an analog to Euler's method for ODEs, and stochastic counterparts to Runge-Kutta methods~\citep{kloeden2013numerical}. As per our previous discussion, the perturbed datapoints of NCSN/DDPM (Eqs.~\eqref{eqn:ncsn} and \eqref{eqn:ddpm}) follow discretized trajectories of forward SDEs (\cref{eqn:ncsn_sde,eqn:ddpm_sde}). For the reverse SDE, we propose to use a closely paralleled discretization strategy, which enjoys simpler implementation and easier adaptation to models with other types of discrete noise scales. Suppose the following is a given discretization of the forward SDE \cref{eqn:forward_sde}:
\begin{align}
    \bfx_{i+1} - \bfx_i = \bfa_i(\bfx_i) + \bfA_i(\bfx_{i})\bfz_i, \label{eqn:discrete_forward}
\end{align}
where $\bfz_i \sim \mcal{N}(\bfzero, \bfI_d)$. We propose to discretize the backward SDE (\cref{eqn:backward_sde}) as below
\begin{align}
    \bfx_{i} - \bfx_{i+1} = -\bfa_{i+1}(\bfx_{i+1}) + \bfA_{i+1}(\bfx_{i+1})\bfA_{i+1}(\bfx_{i+1})\tran \nabla_\bfx \log p(\bfx_{i+1}, t_{i+1}) + \bfA_i(\bfx_{i}) \bfz_i. \label{eqn:discrete_backward}
\end{align}
For NCSN, this gives the following method for sampling
\begin{align}
    \bfx_i = \begin{cases}
        \bfe \sim \mcal{N}(\bfzero, \sM^2\bfI_d), &\quad i = N\label{eqn:ncsn_reverse_diffusion}\\
        \bfx_{i+1} + (\sigma_{i+1}^2 - \sigma_i^2) \bfs_\bftheta(\bfx_{i+1}, t_{i+1}) + \sqrt{\sigma_{i+1}^2 - \sigma_i^2} \bfz_i, &\quad i=0,1,\cdots,N-1.
    \end{cases}
\end{align}
While similarly for DDPM, the discretized reverse SDE is
\begin{align}
    \bfx_i = \begin{cases}
        \bfe \sim \mcal{N}(\bfzero, \bfI_d), &\quad i = N\label{eqn:ddpm_reverse_diffusion}\\
        (2 - \sqrt{1-\beta_{i+1}})\bfx_{i+1} + \beta_{i+1} \bfs_\bftheta(\bfx_{i+1}, t_{i+1}) + \sqrt{\beta_{i+1}}\bfz_i,&\quad i=0,1,\cdots,N-1.
    \end{cases}
\end{align}
We call these new sampling algorithms the \emph{reverse diffusion} sampling method. Note that the original sampling method of DDPM matches \cref{eqn:ddpm_reverse_diffusion} when for all $i$ we have $\beta_i \to 0$, because
\begin{align*}
    &\frac{1}{\sqrt{1-\beta_{i+1}}}(\bfx_i + \beta_{i+1} \bfs_\bftheta) \approx \bigg( 1 + \frac{1}{2}\beta_{i+1} \bigg)(\bfx_i + \beta_{i+1} \bfs_\bftheta) \approx \bigg(1 + \frac{1}{2}\beta_{i+1} \bigg) \bfx_{i} + \beta_{i+1}\bfs_\bftheta \\
    =& \bigg[2 - \bigg(1 - \frac{1}{2}\beta_{i+1}\bigg) \bigg] \bfx_{i} + \beta_{i+1}\bfs_\bftheta \approx (2 - \sqrt{1-\beta_{i+1}})\bfx_{i} + \beta_{i+1}\bfs_\bftheta.
\end{align*}
Therefore, the original sampling method of DDPM is essentially a different discretization to the reverse SDE. However, the derivation of our new reverse diffusion sampler (\cref{eqn:ddpm_reverse_diffusion}) is simpler, and more readily available once a discrete forward process like \cref{eqn:ncsn} or \cref{eqn:ddpm} is given. Empirically, this reverse diffusion sampling process works comparably well or better to the original DDPM sampling method. In fact, for the same DDPM model on CIFAR-10, reverse diffusion achieves an FID score of $3.21\pm 0.02$, while the original sampler achieves $3.24\pm 0.02$ (\cref{tab:compare_samplers})

\subsection{Predictor-corrector samplers}
Different from solving general SDEs, we have extra information that can be readily leveraged to improve the solution. Since we have a score-based model $\bfs_\bftheta(\bfx, t) \approx \nabla_\bfx \log p_t(\bfx)$, we can employ score-based MCMC approaches, such as Langevin MCMC~\citep{parisi1981correlation,grenander1994representations} and HMC~\citep{neal2011mcmc}, to sample from $p_t(\bfx_t)$ directly and correct the solution of a numerical SDE solver. At each time step, the numerical SDE solver gives an estimate of the sample at the next time step, playing the role of a ``predictor''. The score-based MCMC approach corrects the estimated sample using the score-based model, playing the role of a ``corrector''. We therefore name these hybrid sampling algorithms \emph{Predictor-Corrector} (PC) methods.

\begin{figure}
\includegraphics[width=\linewidth]{figures/algorithms.pdf}
\end{figure}

\if0
\algnewcommand{\LineComment}[1]{\Statex \(\triangleright\) #1}
\algrenewcommand\algorithmicindent{0.7em}%
\begin{minipage}[t]{.49\textwidth}
    \begin{algorithm}[H]
           \caption{PC sampling for NCSN}
           \label{alg:ncsn}
            \begin{algorithmic}[1]
               \State $\bfx_N \sim \mcal{N}(\bfzero, \sM^2 \bfI_d)$
               \For{$i=N-1$ {\bfseries to} $0$}
                 \State{$\bfx_i' \gets \bfx_{i+1} + (\sigma_{i+1}^2 - \sigma_i^2) \bfs_\bftheta(\bfx_{i+1}, t_{i+1})$}
                 \State{$\bfz \sim \mcal{N}(\bfzero, \bfI_d)$}
                 \State{$\bfx_i \gets \bfx_i' + \sqrt{\sigma_{i+1}^2 - \sigma_i^2} \bfz$}
                 \For{$j=1$ {\bfseries to} $M$}
                    \State{$\bfz \sim \mcal{N}(\bfzero, \bfI_d)$}
                    \State{$\bfx_{i} \gets \bfx_{i} + \delta_i \bfs_\bftheta(\bfx_{i}, t_{i}) + \sqrt{2\delta_i}\bfz$}
                 \EndFor
               \EndFor
               \State {\bfseries return} $\bfx_0$
            \end{algorithmic}
    \end{algorithm}
\end{minipage}
\begin{minipage}[t]{.49\textwidth}
    \begin{algorithm}[H]
           \caption{PC sampling for DDPM}
           \label{alg:ncsn}
            \begin{algorithmic}[1]
               \State $\bfx_N \sim \mcal{N}(\bfzero, \bfI_d)$
               \For{$i=N-1$ {\bfseries to} $0$}
               \vspace{0.33em}
                 \State{\resizebox{\linewidth}{!}{$\bfx_i' \gets (2 - \sqrt{1-\beta_{i+1}})\bfx_{i+1} + \beta_{i+1} \bfs_\bftheta(\bfx_{i+1}, t_{i+1})$}}\vspace{0.35em}
                 \State{$\bfz \sim \mcal{N}(\bfzero, \bfI_d)$}
                 \State{$\bfx_i \gets \bfx_i' + \sqrt{\beta_{i+1}} \bfz$}
                 \For{$j=1$ {\bfseries to} $M$}
                    \State{$\bfz \sim \mcal{N}(\bfzero, \bfI_d)$}
                    \State{$\bfx_{i} \gets \bfx_{i} + \epsilon_i \bfs_\bftheta(\bfx_{i}, t_{i}) + \sqrt{2\epsilon_i}\bfz$}
                 \EndFor
               \EndFor
               \State {\bfseries return} $\bfx_0$
            \end{algorithmic}
    \end{algorithm}
\end{minipage}
\fi



When using the reverse diffusion sampling method as the predictor, and annealed Langevin MCMC as the corrector, we have Alg.~1 and Alg.~2 for NCSN and DDPM respectively, where $M$ represents the number of Langevin sampling steps per noise scale. In addition, we use $\{\delta_i\}_{i=0}^{N-1}$ and $\{\epsilon_i\}_{i=0}^{N-1}$ to denote step size schedules for Langevin dynamics. In our experiments, we take the schedule of annealed Langevin dynamics in \citet{song2019generative}, but modify it slightly in order to achieve better empirical performance (see Appendix for details). Algs.~1 and 2 generalize the original sampling methods of NCSN and DDPM: We can recover annealed Langevin dynamics for NCSN by removing the predictor part, or regain the reverse diffusion sampling method for DDPM by removing the corrector, which equals the original DDPM sampling method in the limit of small time steps.

\paragraph{Error analysis} The error of sampling with the reverse-time SDE comes from two sources: discretization of the SDE, and estimation of the true scores. We can use a finer discretization and/or a higher-order numerical solver to reduce the discretization error, but this might lead to larger estimation errors since using more discretization steps amounts to evaluating score-based models at more time steps. The estimation errors of the score-based model at multiple time steps can compound. This estimation error can be reduced by incorporating the corrector step, because if the sampler used for the corrector step is accurate (which can be controlled by tuning the step sizes and number of sampling steps of the MCMC), the final samples will only come from the score-based model for the smallest noise scale, and are asymptotically agnostic to the estimation errors of other scores. PC samplers have the benefit of avoiding the accumulation of estimation errors over time.

\paragraph{PC improves performance} We train an NCSN and a DDPM model using the architecture in \cite{ho2020denoising} on CIFAR-10. Results in \cref{tab:compare_samplers} confirm that the reverse diffusion sampling method outperforms the DDPM sampling method. In addition, no matter what type of predictor method is used, adding corrector always gives better performance at the cost of more computation. \todo{results with the same computation.}

\paragraph{Predictor vs. corrector} We conduct an empirical study to demonstrate that in many cases, it is beneficial 
to split computation between the predictor and the corrector, rather than allocating all computation to either the predictor (as done in DDPM) or the corrector (as done in NCSN). As an illustration, we train a score-based model on $256\times 256$ LSUN bedrooms with the SDE of NCSN, and report the results of different computation allocation in \cref{fig:computation}.
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/computation.pdf}
    \caption{Predictor-corrector sampling for LSUN bedrooms. The vertical axis corresponds to the total computation, and the horizontal axis represents the amount of computation allocated to the corrector. Samples are the best when computation is split between the predictor and corrector. \todo{change it to 4x4 grids on both bedrooms and church/celeba-hq. }}
    \label{fig:computation}
\end{figure}

\begin{table}
	\caption{The performance of various samplers applied to NCSN/DDPM models trained on CIFAR-10. Results are averaged over 5 different set of samples. \todo{make this a bar plot instead of a table?}}\label{tab:compare_samplers}
	\centering
	\begin{adjustbox}{max width=\textwidth}
		\begin{tabular}{cccc}
			\Xhline{3\arrayrulewidth} \bigstrut
			Predictor & Corrector & Model & FID \\
			\Xhline{1\arrayrulewidth}\bigstrut
			reverse diffusion	& Yes &	NCSN & $3.60 \pm 0.02$\\
            DDPM sampling & Yes	& NCSN	& $3.62 \pm 0.03$\\
            gradient flow &	Yes	& NCSN	& $3.51 \pm 0.04$\\
            reverse diffuion & No & NCSN & $4.79 \pm 0.07$\\
            gradient flow & No & NCSN & $15.41 \pm 0.15$\\
            DDPM sampling & No & NCSN &	$4.98 \pm 0.06$\\
            reverse diffusion &	Yes & DDPM & $3.18 \pm 0.01$\\
            gradient flow & Yes & DDPM & $3.06 \pm 0.03$\\
            DDPM sampling &	Yes	& DDPM & $3.21 \pm 0.02$\\
            reverse diffuion & No & DDPM & $3.21 \pm 0.02$\\
            gradient flow & No & DDPM & $3.59 \pm 0.04$\\
            DDPM sampling & No & DDPM & $3.24 \pm 0.02$\\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	\end{adjustbox}
\end{table}


\subsection{Probability flow sampling}
The score-based model enables another numerical method for solving the reverse-time SDE. %
For all diffusion processes, there exists a corresponding \emph{deterministic process} whose trajectories induce the same evolution of densities. This deterministic process satisfies an ODE given by deterministic particle flows, which can be derived from the SDE once scores are known. Therefore, we can produce data samples by integrating the associated ODE for the reverse-time SDE, and then collecting endpoints of the resulting trajectories. 

\begin{theorem}[Probability flows for SDEs]
Given the same $p_0(\bfx_0)$, particles flowing according to the following ODE share the same trajectories of densities as the SDE in \cref{eqn:forward_sde}:
\begin{align}
    \ud \bfx_t = \bigg\{\bff(\bfx_t, t) - \frac{1}{2} \nabla \cdot [\bfG(\bfx_t, t)\bfG(\bfx_t, t)\tran] - \frac{1}{2} \bfG(\bfx_t, t)\bfG(\bfx_t, t)\tran \nabla_\bfx \log p_t(\bfx_t)\bigg\} \ud t \label{eqn:flow}.
\end{align}
\end{theorem}

For sample generation, we can either solve the ODE with a fixed discretization strategy (named flow\textsubscript{d}) like the one in NCSN/DDPM, or a black-box integrator with adaptive step sizes and error control (named flow\textsubscript{c}) like in neural ODEs. Both sampling methods can generate reasonable samples with competitive FIDs, as demonstrated in \cref{tab:compare_samplers}. We can explicitly trade accuracy for efficiency with black-box solvers. With a larger error tolerance, the number of function evaluations for a black-box solver can be just $1/10$-th of other sampling methods. \todo{add experimental results here.}

\subsubsection{Exact likelihood computation}
Deterministic probability flows turn our time-dependent score-based model into a neural ODE~\citep{chen2018neural}. Leveraging this connection, we can compute the likelihood of our particle flow dynamics via the instantaneous change of variables formula:
\begin{theorem}[Likelihood of particle flows]
\begin{multline}
\log p_0(\bfx_0) = \log p_T(\bfx_T) + \\
\int \nabla \cdot \bff(\bfx_t, t) - \frac{1}{2} \nabla^2 \cdot [\bfG(\bfx_t, t)\bfG(\bfx_t, t)\tran] - \frac{1}{2} \nabla \cdot [\bfG(\bfx_t, t)\bfG(\bfx_t, t)\tran \nabla_\bfx \log p_t(\bfx_t)]  \ud t
\end{multline}\label{eqn:likelihood}
\end{theorem}
\begin{wraptable}[8]{l}{0.4\textwidth}
\vspace{-2em}
\centering
\caption{NLL on CIFAR-10}\label{tab:bpd}
\begin{adjustbox}{max width=0.4\textwidth}
    \begin{tabular}{l c}
    \toprule
    Model & NLL \\
    \midrule
    DDPM ($L_{\text{simple}}$) & $\leq 3.75$\\
    DDPM (ELBO) & $\leq 3.70$\\
    \midrule
    NCSN cont. & $3.66 \pm 0.0038$\\
    DDPM cont. & $3.40 \pm 0.0040$\\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\end{wraptable}
Here $\nabla^2 := \nabla \cdot \nabla$. The divergence $\nabla \cdot \bfa(\bfx)$ is oftentimes hard to compute, but has an unbiased estimator via Hutchinson's trace estimator~\citep{hutchinson1990stochastic}, \ie, $\nabla \cdot \bfa(\bfx) = \mbb{E}[\bfe \tran \nabla \bfa(\bfx) \bfe]$, where $\bfe$ is a Gaussian or Rademacher random variable, and $\nabla \bfa(\bfx)$ denotes the Jacobian of $\bfa(\bfx)$. Using \cref{eqn:likelihood} and Hutchinson's trace estimator, we can compute the exact likelihood on a test dataset with very small errors~\citep{grathwohl2019scalable}.

We report negative log-likelihoods (NLLs) measured in bits/dim in \cref{tab:bpd}. The likelihoods computed via particle flows are on uniform dequantized data. For DDPM, we obtain better bits/dim compared to the upper bound given by ELBO, since our likelihoods are exact.

\subsubsection{Latent representations}
By integrating \cref{eqn:flow}, we can encode any datapoint $\bfx_0$ into a latent space $\bfx_T$. Decoding can be achieved by integrating a corresponding ODE for the reverse-time SDE. Same as other invertible models such neural ODEs and normalizing flows~\citep{dinh2016density,song2019mintnet}, we can manipulate this latent representation for image editing, such as interpolation, and temperature scaling. \todo{Add experimental results}

There is one special difference from other invertible models: our representation is uniquely identifiable, meaning that with sufficient training data, model capacity, and optimization accuracy, the encoding for a same input always stays the same. This is because our forward SDE, \cref{eqn:forward_sde}, is prescribed without trainable parameters, and its associated particle flow ODE, \cref{eqn:flow}, provides the same trajectories given perfectly estimated scores. \todo{add a quick figure to verify this.}


\section{Controllable generation}
The continuous structure of our framework allows us to not only produce data samples from $p_0(\bfx_0)$, but also control this sampling process for a multitude of other tasks. Let $p_t(\bfx_t \mid \bfy)$ be the posterior distribution of $p_t(\bfx_t)$ given the additional information $\bfy$. We provide a principled method to sample from $p_0(\bfx_0 \mid \bfy)$ at test time for an unconditional score-based model, without re-training it on additional information. The method can be applied to image inpainting, colorization, class-conditional sample generation and others by training a single time-dependent score-based model.


\begin{theorem}[Conditional reverse-time SDE]
Trajectories of the reverse-time SDE
\begin{multline}
\ud \bfx_t = \{\bff(\bfx_t, t) - \nabla \cdot [\bfG(\bfx_t, t) \bfG(\bfx_t,t)\tran] - \bfG(\bfx_t,t)\bfG(\bfx_t,t)\tran  \nabla_\bfx  \log p_t(\bfx_t)\\ - \bfG(\bfx_t,t)\bfG(\bfx_t,t)\tran  \nabla_\bfx  \log p_t(\bfy \mid \bfx_t)\} \ud t + \mbf{G}(\bfx_t, t) \ud \bar{\bfw}_t
\end{multline}
satisfy the marginal probability $p_t(\bfx_t \mid \bfy)$ at time $t$.
\end{theorem}


\subsection{Class-conditional sampling}
When $\bfy$ represents class labels, we can train a time-dependent classifier $p_t(\bfy \mid \bfx_t)$ for class-conditional sampling. Since the forward SDE is tractable, we can easily create a pair of training data $(\bfx_t, \bfy)$ by first sampling $(\bfx_0, \bfy)$ from a dataset and then obtaining $\bfx_t \sim p_{0t}(\bfx_t \mid \bfx_0)$. Afterwards, we may employ a mixture of cross-entropy losses over different time steps, like \cref{eqn:training}, to train the time-dependent classifier $p_t(\bfy \mid \bfx_t)$.

\todo{add pictures}

\subsection{Imputation} 
Imputation is a special case of conditional sampling. Denote by $\Omega(\bfx)$ and $\bar{\Omega}(\bfx)$ the known and unknown dimensions of $\bfx$ respectively, and let $\bff_\Omega(\cdot, t)$ and $\bfG_\Omega(\cdot, t)$ denote $\bff(\cdot, t)$ and $\bfG(\cdot, t)$ restricted to the known dimensions. When $\bff(\cdot, t)$ is element-wise (true for NCSN/DDPM), $\bff_\Omega(\cdot, t)$ denotes the same element-wise function applied only to the known dimensions. When $\bfG(\cdot, t)$ is diagonal (true for NCSN/DDPM), $\bfG_\Omega(\cdot, t)$ is the sub-matrix of known dimensions. 

We aim to sample from $p(\bar{\Omega}(\bfx_0) \mid \Omega(\bfx_0) = \bfy)$. Let $\bfz_t = \Omega(\bfx_t)$. The SDE for $\bfz_t$ can be written as
\begin{align*}
\ud \bfz_t = \bff_\Omega(\bfz_t, t) dt + \bfG_\Omega(\bfz_t, t) \ud \bfw_t,
\end{align*}
The reverse diffusion, given $\Omega(\bfx_0) = \bfy$, is
\begin{align*}
\ud\bfz_t = (\bff_\Omega(\bfz_t, t) - \bfG_\Omega(\bfz_t, t)\bfG_\Omega(\bfz_t, t)\tran \nabla_\bfz \log p_t(\bfz_t \mid \Omega(\bfz_0) = \bfy))\ud t + \bfG_\Omega(\bfz_t, t)\ud\bar{\bfw}_t.
\end{align*}
Although $p_t(\bfz_t \mid \Omega(\bfx_0) = \bfy)$ is in general intractable, it can be approximated by
\begin{align*}
p_t(\bfz_t \mid \Omega(\bfx_0) = \bfy) &= \int p_t(\bfz_t \mid \Omega(\bfx_t), \bfy) p_t(\Omega(\bfx_t) \mid \bfy) \ud \Omega(\bfx_t) \\
&= \mathbb{E}_{p_t(\Omega(\bfx_t) \mid \bfy)}[p_t(\bfz_t \mid \Omega(\bfx_t), \bfy)]\\
&\approx \mathbb{E}_{p_t(\Omega(\bfx_t) \mid \bfy)}[p_t(\bfz_t \mid \Omega(\bfx_t))]\\
&\approx p_t(\bfz_t \mid \Omega'(\bfx_t)),
\end{align*}
where $\Omega'(\bfx_t) \sim p_t(\Omega(\bfx_t) \mid \bfy)$.
Therefore,
\begin{align*}
\nabla_\bfz \log p_t(\bfz_t \mid \Omega(\bfx_0)=\bfy) &\approx \nabla_\bfz \log p_t(\bfz_t \mid \Omega'(\bfx_t)) \\
&= \nabla_\bfz \log p_t([\bfz_t; \Omega'(\bfx_t)]).
\end{align*}

Colorization is a special case of imputation, except for the known data dimensions are coupled. We can decouple these data dimensions with an orthogonal linear transformation, and perform imputation in the transformed space. \todo{include proof-of-concept images.}

==> score sde (v2)_arXiv/abstract.tex <==
\begin{abstract}
Creating noise from data is easy; creating data from noise is generative modeling. We present a stochastic differential equation (SDE) that smoothly transforms a complex data distribution to a known prior distribution by slowly injecting noise, and a corresponding reverse-time SDE that transforms the prior distribution back into the data distribution by slowly removing the noise. 
Crucially, the reverse-time SDE depends only on the time-dependent gradient field (\aka, score) of the perturbed data distribution. By leveraging advances in score-based generative modeling, we can accurately estimate these scores with neural networks, and use numerical SDE solvers to generate samples. We show that this framework encapsulates previous approaches in score-based generative modeling and diffusion probabilistic modeling, allowing for new sampling procedures and new modeling capabilities. In particular, we introduce a predictor-corrector framework to correct errors in the evolution of the discretized reverse-time SDE. We also derive an equivalent neural ODE that samples from the same distribution as the SDE, but additionally enables exact likelihood computation, and improved sampling efficiency. In addition, we provide a new way to solve inverse problems with score-based models, 
as demonstrated with experiments on class-conditional generation, image inpainting, and colorization. Combined with multiple architectural improvements, we achieve record-breaking performance for unconditional image generation on CIFAR-10 with an Inception score of 9.89 and FID of 2.20, a competitive likelihood of 2.99 bits/dim, and demonstrate high fidelity generation of $1024\times 1024$ images for the first time from a score-based generative model.
\end{abstract}

==> score sde (v2)_arXiv/background.tex <==
\section{Background}
\subsection{Denoising score matching with Langevin dynamics (SMLD)}\label{sec:ncsn}
Let $p_{\sigma}(\tilde{\bfx} \mid \bfx) \coloneqq \mcal{N}(\tilde{\bfx}; \bfx, \sigma^2 \bfI)$ be a perturbation kernel, and $p_{\sigma}(\tilde{\bfx}) \coloneqq \int \pd(\bfx) p_{\sigma}(\tilde{\bfx} \mid \bfx) \ud \bfx$, where $\pd(\bfx)$ denotes the data distribution. Consider a sequence of positive noise scales $\sm = \sigma_1 < \sigma_2 < \cdots < \sigma_{N} = \sM$. Typically, $\sm$ is small enough such that $p_{\sm}(\bfx) \approx \pd(\bfx)$, and $\sM$ is large enough such that $p_{\sM}(\bfx) \approx \mcal{N}(\bfx; \bfzero, \sM^2 \bfI)$. \citet{song2019generative} propose to train a Noise Conditional Score Network (NCSN), denoted by $\bfs_\bftheta(\bfx, \sigma)$, with a weighted sum of denoising score matching~\citep{vincent2011connection} objectives:
\begin{align}
\bftheta^* &= \argmin_\bftheta
   \sum_{i=1}^{N} \sigma_i^2  \mbb{E}_{\pd(\bfx)}\mbb{E}_{p_{\sigma_i}(\tilde{\bfx} \mid \bfx)}\big[\norm{ \bfs_\bftheta(\tilde{\bfx}, \sigma_i) - \nabla_{\tilde{\bfx}} \log p_{\sigma_i}(\tilde{\bfx} \mid \bfx)}_2^2 \big]. \label{eqn:ncsn_obj}
\end{align}
Given sufficient data and model capacity, the optimal score-based model $\bfs_{\bftheta^*}(\bfx, \sigma)$ matches $\nabla_\bfx \log p_{\sigma}(\bfx)$ almost everywhere for $\sigma \in \{\sigma_i\}_{i=1}^{N}$. For sampling, \citet{song2019generative} run $M$ steps of Langevin MCMC to get a sample for each $p_{\sigma_i}(\bfx)$ sequentially:
\begin{align}
    \bfx_i^m = \bfx_i^{m-1} + \epsilon_i \bfs_{\bftheta^*}(\bfx_i^{m-1}, \sigma_{i}) + \sqrt{2\epsilon_i} \bfz_{i}^m,\quad m=1,2,\cdots, M,\label{eqn:langevin}
\end{align}
where $\epsilon_i > 0$ is the step size, and $\bfz_i^m$ is standard normal. %
The above is repeated for $i=N, N-1, \cdots, 1$ in turn with $\bfx_{N}^0 \sim \mcal{N}(\bfx \mid \bfzero, \sM^2 \bfI)$ and $\bfx_i^0 = \bfx_{i+1}^{M}$ when $i < N$. As $M \to \infty$ and $\epsilon_i \to 0$ for all $i$, $\bfx_1^M$ becomes an exact sample from $p_{\sm}(\bfx) \approx \pd(\bfx)$ under some regularity conditions.

\subsection{Denoising diffusion probabilistic models (DDPM)}\label{sec:ddpm}
\citet{sohl2015deep,ho2020denoising} consider a sequence of positive noise scales $0 < \beta_1, \beta_2, \cdots, \beta_N < 1$. For each training data point $\bfx_0 \sim \pd(\bfx)$, a discrete Markov chain $\{ \bfx_0, \bfx_1, \cdots, \bfx_N \}$ is constructed such that $p(\bfx_{i} \mid \bfx_{i-1}) = \mcal{N}(\bfx_{i} ; \sqrt{1-\beta_i} \bfx_{i-1}, \beta_i \bfI)$, and therefore $p_{\alpha_i}(\bfx_i \mid \bfx_0) = \mcal{N}(\bfx_i ;\sqrt{\alpha_i} \bfx_0, (1-\alpha_i)\bfI)$, where $\alpha_i \coloneqq \prod_{j=1}^i (1-\beta_j)$. Similar to SMLD, we can denote the perturbed data distribution as $p_{\alpha_i}(\tilde{\bfx}) \coloneqq \int p_\text{data}(\bfx) p_{\alpha_i}(\tilde{\bfx} \mid \bfx) \ud \bfx$. The noise scales are prescribed such that %
$\bfx_N$ is approximately distributed according to $\mcal{N}(\bfzero, \bfI)$. A variational Markov chain in the reverse direction is parameterized with $p_\bftheta(\bfx_{i-1} | \bfx_{i}) = \mcal{N}(\bfx_{i-1}; \frac{1}{\sqrt{1-\beta_i}} (\bfx_i + \beta_i \bfs_\bftheta(\bfx_i, i)), \beta_i \bfI)$, and trained with a re-weighted variant of the evidence lower bound (ELBO):
\begin{align}
\bftheta^* &= \argmin_\bftheta
    \sum_{i=1}^{N} (1-\alpha_i) \mbb{E}_{\pd(\bfx)}\mbb{E}_{p_{\alpha_i}(\tilde{\bfx} \mid \bfx)}[\norm{ \bfs_\bftheta(\tilde{\bfx}, i) - \nabla_{\tilde{\bfx}} \log p_{\alpha_i}(\tilde{\bfx} \mid \bfx)}_2^2]. \label{eqn:ddpm_obj}
\end{align}
After solving \cref{eqn:ddpm_obj} to get the optimal model $\bfs_{\bftheta^*}(\bfx, i)$, samples can be generated by starting from $\bfx_N \sim \mcal{N}(\bfzero, \bfI)$ and following the estimated reverse Markov chain as below
\begin{align}
    \bfx_{i-1} = \frac{1}{\sqrt{1-\beta_i}} (\bfx_i + \beta_i \bfs_{\bftheta^*}(\bfx_i, i)) + \sqrt{\beta_i}\bfz_i, \quad i=N, N-1, \cdots, 1. \label{eqn:ddpm_sampling}
\end{align}
We call this method \emph{ancestral sampling}, since it amounts to performing ancestral sampling from the graphical model $\prod_{i=1}^N p_\bftheta(\bfx_{i-1} \mid \bfx_i)$. The objective \cref{eqn:ddpm_obj} described here is $L_{\text{simple}}$ in \citet{ho2020denoising}, written in a form to expose more similarity to \cref{eqn:ncsn_obj}. 
Like \cref{eqn:ncsn_obj}, \cref{eqn:ddpm_obj} is also a weighted sum of denoising score matching objectives, which implies that the optimal model, $\bfs_{\bftheta^*}(\tilde{\bfx}, i)$, matches the score of the perturbed data distribution, $\nabla_\bfx \log p_{\alpha_i}(\bfx)$. Notably, the weights of the $i$-th summand in \cref{eqn:ncsn_obj} and \cref{eqn:ddpm_obj}, namely $\sigma_i^2$ and $(1-\alpha_i)$, are related to corresponding perturbation kernels in the same functional form: $\sigma_i^2 \propto 1/\mbb{E}[\norm{\nabla_\bfx \log p_{\sigma_i}(\tilde{\bfx} \mid \bfx)}_2^2]$ and $(1-\alpha_i) \propto 1/\mbb{E}[\norm{\nabla_\bfx \log p_{\alpha_i}(\tilde{\bfx} \mid \bfx)}_2^2]$. %



==> score sde (v2)_arXiv/conclusion.tex <==
\section{Conclusion}
We presented a framework for score-based generative modeling based on SDEs. Our work enables a better understanding of existing approaches,  new sampling algorithms, exact likelihood computation, uniquely identifiable encoding, latent code manipulation, and brings new conditional generation abilities to the family of score-based generative models.

While our proposed sampling approaches improve results and enable more efficient sampling, they remain slower at sampling than GANs~\citep{goodfellow2014generative} on the same datasets. Identifying ways of combining the stable learning of score-based generative models with the fast sampling of implicit models like GANs remains an important research direction. Additionally, the breadth of samplers one can use when given access to score functions introduces a number of hyper-parameters. Future work would benefit from improved methods to automatically select and tune these hyper-parameters, as well as more extensive investigation on the merits and limitations of various samplers.

\subsubsection*{Acknowledgements}
We would like to thank Nanxin Chen, Ruiqi Gao, Jonathan Ho, Kevin Murphy, Tim Salimans and Han Zhang for their insightful discussions during the course of this project. This research was partially supported by NSF (\#1651565, \#1522054, \#1733686),
ONR (N00014\-19\-1\-2145), AFOSR (FA9550\-19\-1\-0024), and TensorFlow Research Cloud. Yang Song was partially supported by the Apple PhD Fellowship in AI/ML.

==> score sde (v2)_arXiv/cond_gen.tex <==
\section{Controllable generation}
The continuous structure of our framework allows us to not only produce data samples from $p_0$, but also from $p_0(\bfx(0) \mid \bfy)$ if $p_t(\bfy \mid \bfx(t))$ is known. %
Given a forward SDE as in \cref{eqn:forward_sde}, we can sample from $p_t(\bfx(t) \mid \bfy)$ by starting from $p_T(\bfx(T) \mid \bfy)$ and solving a conditional reverse-time SDE:
\begin{align}
\ud \bfx = \{\bff(\bfx, t) - g(t)^2[ \nabla_\bfx  \log p_t(\bfx)+  \nabla_{\bfx}  \log p_t(\bfy \mid \bfx)]\} \ud t + g(t) \ud \bar{\bfw}.\label{eqn:cond_sde}
\end{align}
In general, we can use \cref{eqn:cond_sde} to solve a large family of \emph{inverse problems} with score-based generative models, once given an estimate of the gradient of the forward process, $\nabla_\bfx \log p_t(\bfy \mid \bfx(t) )$. In some cases, it is possible to train a separate model to learn the forward process $\log p_t(\bfy \mid \bfx(t))$ and compute its gradient. Otherwise, we may estimate the gradient with heuristics and domain knowledge. In \cref{app:inverse_prob}, we provide a broadly applicable method for obtaining such an estimate without the need of training auxiliary models.

We consider three applications of controllable generation with this approach: class-conditional generation, image imputation and colorization. When $\bfy$ represents class labels, we can train a time-dependent classifier $p_t(\bfy \mid \bfx(t))$ for class-conditional sampling. Since the forward SDE is tractable, we can easily create training data $(\bfx(t), \bfy)$ for the time-dependent classifier
by first sampling $(\bfx(0), \bfy)$ from a dataset, and then sampling $\bfx(t) \sim p_{0t}(\bfx(t) \mid \bfx(0))$. Afterwards, we may employ a mixture of cross-entropy losses over different time steps, like \cref{eqn:training}, to train the time-dependent classifier $p_t(\bfy \mid \bfx(t))$. We provide class-conditional CIFAR-10 samples in \cref{fig:cond_gen} (left), and relegate more details and results to \cref{app:cond_gen}.

Imputation is a special case of conditional sampling.
Suppose we have an incomplete data point $\bfy$ where only some subset, $\Omega(\bfy)$ is known. Imputation amounts to sampling from $p(\bfx(0) \mid \Omega(\bfy))$, which we can accomplish using an unconditional model (see \cref{app:imputation}). Colorization is a special case of imputation, except that the known data dimensions are coupled. We can decouple these data dimensions with an orthogonal linear transformation, and perform imputation in the transformed space (details in \cref{app:colorization}). \cref{fig:cond_gen} (right) shows results for inpainting and colorization achieved with unconditional time-dependent score-based models.


\begin{figure}
    \centering
    \includegraphics[width=0.327\linewidth, trim=5 0 7 0, clip, valign=c]{figures/cond_gen_line.png}
    \includegraphics[width=0.66\linewidth, valign=c]{figures/inpaint_colorization.jpg}
    \caption{\textit{Left}: Class-conditional samples on $32\times 32$ CIFAR-10. Top four rows are automobiles and bottom four rows are horses. \textit{Right:} Inpainting (top two rows) and colorization (bottom two rows) results on $256\times 256$ LSUN. First column is the original image, second column is the masked/gray-scale image, remaining columns are sampled image completions or colorizations.}
    \label{fig:cond_gen}
\end{figure}


==> score sde (v2)_arXiv/intro.tex <==
\section{Introduction}



Two successful classes of probabilistic generative models involve sequentially corrupting training data with slowly increasing noise, and then learning to reverse this corruption in order to form a generative model of the data. 
\emph{Score matching with Langevin dynamics} (SMLD)~\citep{song2019generative} %
estimates the \emph{score} (\ie, the gradient of the log probability density with respect to data) at each noise scale, and then uses Langevin dynamics to sample from a sequence of decreasing noise scales during generation. 
\emph{Denoising diffusion probabilistic modeling} (DDPM)~\citep{sohl2015deep,ho2020denoising} trains a sequence of probabilistic models to reverse each step of the noise corruption, 
using knowledge of the functional form of the reverse distributions to make training tractable. 
For continuous state spaces, the DDPM training objective implicitly computes 
scores at each noise scale. 
We therefore refer to these two model classes together as \emph{score-based generative models}. %

Score-based generative models, and related techniques \citep{bordes2017learning,goyal2017variational, du2019implicit}, have proven effective at generation of images~\citep{song2019generative,song2020improved,ho2020denoising}, audio~\citep{chen2020wavegrad,kong2020diffwave}, graphs~\citep{niu20a}, and shapes~\citep{ShapeGF}. To enable new sampling methods and further extend the capabilities of score-based generative models, we propose a unified framework that generalizes previous approaches through the lens of stochastic differential equations (SDEs).%



\begin{SCfigure}
    \centering
    \caption{{\bf Solving a reverse-time SDE yields a score-based generative model.} Transforming data to a simple noise distribution can be accomplished with a continuous-time SDE. This SDE can be reversed if we know the score of the distribution at each intermediate time step, $\nabla_\bfx \log p_t(\bfx)$. }
    \includegraphics[width=0.65\linewidth, trim=105 0 110 0, clip]{figures/diffusion_schematic.pdf}
    \label{fig:teaser}
\end{SCfigure}

Specifically, instead of perturbing data with a finite number of noise distributions, we consider a continuum of distributions that evolve over time according to a diffusion process. This process progressively diffuses a data point into random noise, and is given by a prescribed SDE that does not depend on the data and has no trainable parameters. 
By reversing this process, we can smoothly mold random noise into data for sample generation. Crucially, this reverse process satisfies a reverse-time SDE~\citep{Anderson1982-ny}, which can be derived from the forward SDE given the score of the marginal probability densities as a function of time. We can therefore approximate the reverse-time SDE by training a time-dependent neural network to estimate the scores, and then produce samples using numerical SDE solvers. Our key idea is summarized in \cref{fig:teaser}.

Our proposed framework has several theoretical and practical contributions: %

\textbf{Flexible sampling and likelihood computation:}~ We can employ any general-purpose SDE solver to integrate the reverse-time SDE for sampling. In addition, we propose two special methods not viable for general SDEs: (i) Predictor-Corrector (PC) samplers that combine numerical SDE solvers with score-based MCMC approaches, such as Langevin MCMC~\citep{parisi1981correlation} and HMC~\citep{neal2011mcmc}; and (ii) deterministic samplers based on the probability flow ordinary differential equation (ODE). The former \emph{unifies and improves} over existing sampling methods for score-based models. The latter allows for \emph{fast adaptive sampling} via black-box ODE solvers, \emph{flexible data manipulation} via latent codes, a \emph{uniquely identifiable encoding}, and notably, \emph{exact likelihood computation}.

\textbf{Controllable generation:}~ We can modulate the generation process by conditioning on information not available during training, because the conditional reverse-time SDE can be efficiently estimated from \emph{unconditional} scores. This enables applications such as class-conditional generation, image inpainting, colorization and other inverse problems, all achievable using a single unconditional score-based model without re-training.


\textbf{Unified framework:}~ Our framework provides a unified way to explore and tune various SDEs for improving score-based generative models.
The methods of SMLD and DDPM can be amalgamated into our framework as discretizations of two separate SDEs. 
Although DDPM~\citep{ho2020denoising} was recently reported to achieve higher sample quality than SMLD~\citep{song2019generative,song2020improved}, we show that with better architectures and new sampling algorithms allowed by our framework, the latter can catch up---it achieves new state-of-the-art Inception score (9.89) and FID score (2.20) on CIFAR-10, as well as high-fidelity generation of $1024\times 1024$ images for the first time from a score-based model. In addition, we propose a new SDE under our framework that achieves a likelihood value of 2.99 bits/dim on uniformly dequantized CIFAR-10 images, setting a new record on this task.



==> score sde (v2)_arXiv/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> score sde (v2)_arXiv/method.tex <==
\section{Score-based generative modeling with SDEs}
Perturbing data with multiple noise scales is at the crux of the success of previous methods. We propose to generalize this idea further to an infinite number of noise scales, such that perturbed data distributions evolve according to an It\^{o} process as the noise intensifies. %

Note that when using a total of $N$ noise scales, each perturbation kernel $p_{\sigma_i}(\bfx \mid \bfx_0)$ in \cref{sec:ncsn} corresponds to the marginal distribution of $\bfx_i$ in the following Markov chain:
\begin{align}
\bfx_i = \bfx_{i-1} + \sqrt{\sigma_{i}^2 - \sigma_{i-1}^2} \bfz_i, \quad i=1,\cdots,N \label{eqn:ncsn},
\end{align}
where $\bfz_i \sim \mcal{N}(\bfzero, \bfI)$, and we have introduced $\sigma_0 = 0$ to simplify the equation. Let $r \triangleq (\nicefrac{\sm}{\sM})^2$. Because $\{\sigma_i\}_{i=1}^N$ is a geometric sequence, we have $\sigma_i = \sm r^{\frac{i-1}{2(N-1)}}$. In the limit of $N \to \infty$, the Markov chain $\{\bfx_i\}_{i=1}^N$ becomes a continuous process $\bfx(t)$, where we use a continuous time variable $t \in [0, 1]$ for indexing, rather than an integer $i \in \{1, 2, \cdots, N\}$. Let $\Delta t = \frac{1}{N-1}$, and $\bfx(\frac{i-1}{N-1}) = \bfx_i$. As $\Delta t \to 0$, \cref{eqn:ncsn} can be written as the following for $t \in \{\frac{1}{N-1}, \frac{2}{N-1}, \cdots, 1\}$ via Taylor expansion:
\begin{align*}
    \bfx(t) = \bfx(t-\Delta t) + \sm \sqrt{r^t - r^{t-\Delta t}}\bfz_i \approx \bfx(t-\Delta t) + \sm \sqrt{(r^{t-\Delta t}\ln r) \Delta t}~\bfz(t),
\end{align*}
and in the limit of $\Delta t = 0$, it converges to the following SDE for $t \in [0,1]$:
\begin{align}
\ud \bfx = \sm \bigg( \frac{\sM}{\sm} \bigg)^t \sqrt{2 \log \frac{\sM}{\sm}}\ud \bfw, \label{eqn:ncsn_sde}
\end{align}
where $\bfw$ is the standard Wiener process. Likewise for perturbation kernels $\{p_{\alpha_i}(\bfx \mid \bfx_0)\}_{i=1}^N$ in \cref{sec:ddpm}, the discrete Markov chain is
\begin{align}
    \bfx_i = \sqrt{1-\beta_{i}} \bfx_{i-1} + \sqrt{\beta_{i}} \bfz_i, \quad i=1,\cdots,N. \label{eqn:ddpm}
\end{align}
and the corresponding SDE can be obtained through a similar analysis (see Appendix):
\begin{align}
\ud \bfx = -\frac{1}{2}(\bbetam + t(\bbetaM - \bbetam)) \bfx(t) \ud t + \sqrt{\bbetam + t(\bbetaM - \bbetam)} \ud \bfw, \label{eqn:ddpm_sde}
\end{align}
where $\bbetam = (N-1) \betam$ and $\bbetaM = (N-1) \betaM$.

So far, we have demonstrated that the noise perturbations used in \citet{song2019generative} and \citet{ho2020denoising} both correspond to discretizations of SDEs. The SDE of \cref{eqn:ddpm_sde} yields a process with constant variance, as long as $p(\bfx_0)$ has variance one (proof in Appendix). In contrast, the SDE of \cref{eqn:ncsn_sde} always gives a process with exploding variance. Due to this difference, we hereafter refer to \cref{eqn:ncsn_sde} the variance exploding (VE) SDE, and \cref{eqn:ddpm_sde} the variance preserving (VP) SDE.

In general, we can consider noise peturbations that evolve according to any SDE:
\begin{align}
    \ud \bfx = \bff(\bfx(t), t) \ud t + \mbf{G}(\bfx(t), t) \ud \bfw. \label{eqn:forward_sde}
\end{align}
Here $\bff(\cdot, t): \mbb{R}^d \to \mbb{R}^d$ is a vector-valued function called the \emph{drift} coefficient, $\mbf{G}(\cdot, t): \mbb{R}^d \to \mbb{R}^{d\times d}$ is a matrix-valued function known as the \emph{dispersion} coefficient. %
In this work we follow the It\^{o} interpretation of SDEs. Under some regularity conditions~\citep{oksendal2003stochastic}, the solution to an SDE is an It\^{o} diffusion process $\bfx(t)$. We denote by $p_t(\bfx)$ the (marginal) probability density of $\bfx(t)$, and use $p_{st}(\bfx(t) \mid \bfx(s))$ to denote the transition kernel from time $s$ to $t$.%

We can use a continuous diffusion process to gradually diffuse an unknown distribution $p_0(\bfx_0)$, for which we have a dataset of \iid samples, to a known prior distribution $p_T(\bfx_T)$, for which we have a tractable form and can easily generate samples. 



By starting from $p_T(\bfx_T)$ and reversing the diffusion process, we can obtain $p_0(\bfx_0)$. This reverse process should yield the same trajectory of marginal probability densities $\{p_t(\bfx)\}_{t=0}^T$ as the forward SDE (\cref{eqn:forward_sde}), except that the evolution of $p_t(\bfx)$ is in the opposite time direction. A remarkable result from~\citet{Anderson1982-ny} states that the reverse of a diffusion process is also a diffusion process, running backwards in time. Moreover, the reverse diffusion process can be derived from the forward process, once the score of each marginal distribution, $\nabla_\bfx \log p_t(\bfx^t)$, is known for all $t$.
\begin{theorem}[\citet{Anderson1982-ny}, informal]\label{thm:reverse_sde}
The reverse process to \cref{eqn:forward_sde} is given by
\begin{align}
    \resizebox{0.935\textwidth}{!}{$\displaystyle\ud \bfx_t = \{\bff(\bfx_t, t) - \nabla \cdot [\bfG(\bfx_t, t) \bfG(\bfx_t,t)\tran] - \bfG(\bfx_t,t)\bfG(\bfx_t,t)\tran  \nabla_\bfx  \log p_t(\bfx_t)\} \ud t + \mbf{G}(\bfx_t, t) \ud \bar{\bfw}_t$},\label{eqn:backward_sde}
\end{align}
where $\{\bar{\bfw}_t\}_{t=T}^0$ is a standard Wiener process when time flows backwards from $T$ to $0$.\footnote{See Appendix for a rigorous statement.}
\end{theorem}
Throughout the paper we define $\nabla\cdot \mbf{F}(\bfx) := (\nabla \cdot \bff^1(\bfx), \nabla\cdot \bff^2(\bfx), \cdots, \nabla\cdot \bff^d(\bfx))\tran$ for a matrix-valued function $\mbf{F}(\bfx) := (\bff^1(\bfx), \bff^2(\bfx), \cdots, \bff^d(\bfx))\tran$. \cref{thm:reverse_sde} implies that the reverse diffusion is completely determined by the drift and dispersion coefficients of the forward process, as well as the \textbf{score} of its marginal probability density at each time step. Using \cref{thm:reverse_sde}, we can easily reverse \cref{eqn:forward_sde} to get samples from $p_0(\bfx_0)$, by simulating the trajectories of \cref{eqn:backward_sde}. The sampling procedure only requires 1) \textbf{score estimation} to obtain $\nabla_\bfx \log p_t(\bfx)$ of the forward SDE (\cref{eqn:forward_sde}), and 2) a \textbf{numerical SDE solver} to integrate the reverse-time SDE (\cref{eqn:backward_sde}).

\section{Estimating scores of the SDE}
The score of a distribution can be estimated by training a score-based model on samples with score matching~\citep{hyvarinen2005estimation, song2019sliced, song2019generative}. To estimate $\nabla_\bfx \log p_t(\bfx)$ with this approach, we shall choose a forward SDE (\cref{eqn:forward_sde}) whose perturbation kernel $p_{0t}(\bfx_t \mid \bfx_0)$ is solvable, so that we can easily generate training data from $p_t(\bfx)$ given data samples of $p_0(\bfx)$. One such example is linear SDEs.
\begin{proposition}[\citet{sarkka2019applied}, exact solution to linear SDEs]\label{prop:linear}
When the drift and dispersion coefficients in \cref{eqn:forward_sde} possess the form $\bff(\bfx_t, t) = \bfF(t)\bfx_t + \bfu(t)$ and $\bfG(\bfx_t, t) = \bfL(t)$, the transition kernel is $p_{0t}(\bfx_t \mid \bfx_0) = \mcal{N}(\bfx_t \mid \bfm(t), \bfsigma(t))$, where $\bfm(t)$ and $\bfsigma(t)$ are obtained by solving the following linear ODEs:
\begin{gather*}
\frac{\ud \bfm(t)}{\ud t} = \bfF(t)\bfm(t) + \bfu(t), \quad \bfm(0) = \bfx_0,\\
\frac{\ud \bfsigma(t)}{\ud t} = \bfF(t)\bfsigma(t) + \bfsigma(t)\bfF(t) + \bfL(t) \bfL(t)\tran, \quad \bfsigma(0) = \bfzero.
\end{gather*}
\end{proposition}
Typically we only have a dataset for $p_0(\bfx_0)$, but when an SDE is linear, we can employ the perturbation kernel provided by \cref{prop:linear} to directly obtain training data from $p_t(\bfx_t)$. Specifically, we first randomly select a data point $\bfx_0 \sim p_0(\bfx_0)$, and then draw $\bfx_t$ from the perturbation kernel $p_{0t}(\bfx_t \mid \bfx_0)$. Based on samples from $p_t(\bfx_t)$, we can use the following (infinite) mixture of score matching objectives to train a time-dependent score-based model $\bfs_\bftheta(\bfx, t)$ parameterized by $\bftheta$:
\begin{align}
    \min_\bftheta \mbb{E}_{\bfx_0 \sim p_0(\bfx_0)}\mbb{E}_{t\sim \mcal{U}(0, T)} \mbb{E}_{\bfx_t \sim p_{0t}(\bfx \mid \bfx_0)}[\lambda(t) \mcal{L}_{\text{SM}}(\bfs_\bftheta(\bfx_t, t), \bfx_0, \bfx_t)], \label{eqn:training}
\end{align}
where $\lambda: [0, T] \to \mbb{R}_{>0}$ is a positive weighting function, %
$\mcal{U}(0, T)$ denotes a uniform distribution over $[0, T]$, and $\mcal{L}_{\text{SM}}$ is a score matching loss function. With sufficient data, model capacity, and optimization accuracy, score matching ensures that the optimal solution to \cref{eqn:training}, denoted by $\bfs_{\bftheta^\ast}(\bfx, t)$, equals $\nabla_\bfx \log p_t(\bfx)$ for almost all $\bfx$ and $t$. Typical examples of $\mcal{L}_{\text{SM}}$ include denoising score matching (DSM,~\citet{vincent2011connection}), which can be written as 
\begin{align}
    \mathcal{L}_{\text{SM}} := \norm{\bfs_\bftheta(\bfx_t, t) - \nabla_{\bfx_t}\log p_{0t}(\bfx_t \mid \bfx_0)}_2^2. \label{eqn:dsm}
\end{align}
Other alternatives for $\mcal{L}_{\text{SM}}$ include sliced score matching~\citep{song2019sliced} and finite-difference score matching~\citep{pang2020efficient}.

\begin{figure}
    \centering
    \includegraphics[width=0.333\linewidth]{figures/NCSN_var.pdf}%
    \includegraphics[width=0.32\linewidth]{figures/ddpm_mean.pdf}%
    \includegraphics[width=0.32\linewidth]{figures/ddpm_var.pdf}
    \caption{Comparison of discrete-time perturbation kernels vs. continuous ones. \textbf{Left} compares the variance of perturbation kernels at different time steps on NCSN; \textbf{middle} compares the mean coefficients (the ratio of the mean to $\bfxd$) of perturbation kernels on DDPM; and \textbf{right} compares the variance of perturbation kernels on DDPM. }
    \label{fig:discretization}
\end{figure}

The training objectives of NCSN and DDPM can be unified as discretized approximations to \cref{eqn:training} when $\mcal{L}_{\text{SM}}$ is denoising score matching (\cref{eqn:dsm}). Using \cref{prop:linear}, we can analytically compute the perturbation kernels induced by the SDE of NCSN and DDPM. For NCSN, we have
\begin{align}
    p(\bfx_t \mid \bfxd) = \mcal{N}\bigg(\bfx_t; \bfxd, \sm^2 \bigg(\frac{\sM}{\sm} \bigg)^{2t}\bfI_d\bigg), \label{eqn:ncsn_sde_perturb}
\end{align}
while for DDPM,
\begin{align}
    p(\bfx_t \mid \bfxd) = \mcal{N}\bigg(\bfx_t ; e^{-\frac{1}{2}\bbetam t - \frac{1}{4}t^2 (\bbetaM-\bbetam)}\bfxd , \bfI_d - \beta_0 e^{\frac{1}{2}t(t-2)\bbetam-\frac{1}{2}t^2\bbetaM}\bfI_d\bigg).\label{eqn:ddpm_sde_perturb}
\end{align}
The original perturbation kernels $q_{\sigma_i}(\bfx \mid \bfxd)$ and $q_{\beta_i}(\bfx \mid \bfxd)$ for NCSN/DDPM are discretizations of \cref{eqn:ncsn_sde_perturb,eqn:ddpm_sde_perturb} at time steps $\{0, \nicefrac{1}{N-1}, \cdots, \nicefrac{N-2}{N-1}, 1\}$. 
\cref{fig:discretization} shows the near perfect agreement of discrete-time and continuous-time kernels when the number of noise scales $N$ is large. 

Our training method generalizes the original ones in NCSN/DDPM to an infinite number of noise scales, allowing flexible discretization and variable number of noise scales for sampling.





\section{Solving the reverse SDE}
After training a time-dependent score-based model, we can use it to construct the reverse SDE and then solve it to generate samples from $p_0(\bfx_0)$. Crucially, the additional knowledge of scores enables special numerical methods not applicable to general SDEs. These new methods not only provide better sample quality and efficiency, but also allow for exact likelihood computation, flexible manipulation of latent representations, and uniquely identifiable encoding/compression.

\subsection{General numerical solvers}
Numerical solvers provide approximate samples of trajectories from SDEs. Many general methods exist for the numerical integration of SDEs, based on different discretization and approximation strategies. Examples include Euler-Maruyama, an analog to Euler's method for ODEs, and stochastic counterparts to Runge-Kutta methods~\citep{kloeden2013numerical}. As per our previous discussion, the perturbed datapoints of NCSN/DDPM (Eqs.~\eqref{eqn:ncsn} and \eqref{eqn:ddpm}) follow discretized trajectories of forward SDEs (\cref{eqn:ncsn_sde,eqn:ddpm_sde}). For the reverse SDE, we propose to use a closely paralleled discretization strategy, which enjoys simpler implementation and easier adaptation to models with other types of discrete noise scales. Suppose the following is a given discretization of the forward SDE \cref{eqn:forward_sde}:
\begin{align}
    \bfx_{i+1} - \bfx_i = \bfa_i(\bfx_i) + \bfA_i(\bfx_{i})\bfz_i, \label{eqn:discrete_forward}
\end{align}
where $\bfz_i \sim \mcal{N}(\bfzero, \bfI_d)$. We propose to discretize the backward SDE (\cref{eqn:backward_sde}) as below
\begin{align}
    \bfx_{i} - \bfx_{i+1} = -\bfa_{i+1}(\bfx_{i+1}) + \bfA_{i+1}(\bfx_{i+1})\bfA_{i+1}(\bfx_{i+1})\tran \nabla_\bfx \log p(\bfx_{i+1}, t_{i+1}) + \bfA_i(\bfx_{i}) \bfz_i. \label{eqn:discrete_backward}
\end{align}
For NCSN, this gives the following method for sampling
\begin{align}
    \bfx_i = \begin{cases}
        \bfe \sim \mcal{N}(\bfzero, \sM^2\bfI_d), &\quad i = N\label{eqn:ncsn_reverse_diffusion}\\
        \bfx_{i+1} + (\sigma_{i+1}^2 - \sigma_i^2) \bfs_\bftheta(\bfx_{i+1}, t_{i+1}) + \sqrt{\sigma_{i+1}^2 - \sigma_i^2} \bfz_i, &\quad i=0,1,\cdots,N-1.
    \end{cases}
\end{align}
While similarly for DDPM, the discretized reverse SDE is
\begin{align}
    \bfx_i = \begin{cases}
        \bfe \sim \mcal{N}(\bfzero, \bfI_d), &\quad i = N\label{eqn:ddpm_reverse_diffusion}\\
        (2 - \sqrt{1-\beta_{i+1}})\bfx_{i+1} + \beta_{i+1} \bfs_\bftheta(\bfx_{i+1}, t_{i+1}) + \sqrt{\beta_{i+1}}\bfz_i,&\quad i=0,1,\cdots,N-1.
    \end{cases}
\end{align}
We call these new sampling algorithms the \emph{reverse diffusion} sampling method. Note that the original sampling method of DDPM matches \cref{eqn:ddpm_reverse_diffusion} when for all $i$ we have $\beta_i \to 0$, because
\begin{align*}
    &\frac{1}{\sqrt{1-\beta_{i+1}}}(\bfx_i + \beta_{i+1} \bfs_\bftheta) \approx \bigg( 1 + \frac{1}{2}\beta_{i+1} \bigg)(\bfx_i + \beta_{i+1} \bfs_\bftheta) \approx \bigg(1 + \frac{1}{2}\beta_{i+1} \bigg) \bfx_{i} + \beta_{i+1}\bfs_\bftheta \\
    =& \bigg[2 - \bigg(1 - \frac{1}{2}\beta_{i+1}\bigg) \bigg] \bfx_{i} + \beta_{i+1}\bfs_\bftheta \approx (2 - \sqrt{1-\beta_{i+1}})\bfx_{i} + \beta_{i+1}\bfs_\bftheta.
\end{align*}
Therefore, the original sampling method of DDPM is essentially a different discretization to the reverse SDE. However, the derivation of our new reverse diffusion sampler (\cref{eqn:ddpm_reverse_diffusion}) is simpler, and more readily available once a discrete forward process like \cref{eqn:ncsn} or \cref{eqn:ddpm} is given. Empirically, this reverse diffusion sampling process works comparably well or better to the original DDPM sampling method. In fact, for the same DDPM model on CIFAR-10, reverse diffusion achieves an FID score of $3.21\pm 0.02$, while the original sampler achieves $3.24\pm 0.02$ (\cref{tab:compare_samplers})

\subsection{Predictor-corrector samplers}
Different from solving general SDEs, we have extra information that can be readily leveraged to improve the solution. Since we have a score-based model $\bfs_\bftheta(\bfx, t) \approx \nabla_\bfx \log p_t(\bfx)$, we can employ score-based MCMC approaches, such as Langevin MCMC~\citep{parisi1981correlation,grenander1994representations} and HMC~\citep{neal2011mcmc}, to sample from $p_t(\bfx_t)$ directly and correct the solution of a numerical SDE solver. At each time step, the numerical SDE solver gives an estimate of the sample at the next time step, playing the role of a ``predictor''. The score-based MCMC approach corrects the estimated sample using the score-based model, playing the role of a ``corrector''. We therefore name these hybrid sampling algorithms \emph{Predictor-Corrector} (PC) methods.

\begin{figure}
\includegraphics[width=\linewidth]{figures/algorithms.pdf}
\end{figure}

\if0
\algnewcommand{\LineComment}[1]{\Statex \(\triangleright\) #1}
\algrenewcommand\algorithmicindent{0.7em}%
\begin{minipage}[t]{.49\textwidth}
    \begin{algorithm}[H]
           \caption{PC sampling for NCSN}
           \label{alg:ncsn}
            \begin{algorithmic}[1]
               \State $\bfx_N \sim \mcal{N}(\bfzero, \sM^2 \bfI_d)$
               \For{$i=N-1$ {\bfseries to} $0$}
                 \State{$\bfx_i' \gets \bfx_{i+1} + (\sigma_{i+1}^2 - \sigma_i^2) \bfs_\bftheta(\bfx_{i+1}, t_{i+1})$}
                 \State{$\bfz \sim \mcal{N}(\bfzero, \bfI_d)$}
                 \State{$\bfx_i \gets \bfx_i' + \sqrt{\sigma_{i+1}^2 - \sigma_i^2} \bfz$}
                 \For{$j=1$ {\bfseries to} $M$}
                    \State{$\bfz \sim \mcal{N}(\bfzero, \bfI_d)$}
                    \State{$\bfx_{i} \gets \bfx_{i} + \delta_i \bfs_\bftheta(\bfx_{i}, t_{i}) + \sqrt{2\delta_i}\bfz$}
                 \EndFor
               \EndFor
               \State {\bfseries return} $\bfx_0$
            \end{algorithmic}
    \end{algorithm}
\end{minipage}
\begin{minipage}[t]{.49\textwidth}
    \begin{algorithm}[H]
           \caption{PC sampling for DDPM}
           \label{alg:ncsn}
            \begin{algorithmic}[1]
               \State $\bfx_N \sim \mcal{N}(\bfzero, \bfI_d)$
               \For{$i=N-1$ {\bfseries to} $0$}
               \vspace{0.33em}
                 \State{\resizebox{\linewidth}{!}{$\bfx_i' \gets (2 - \sqrt{1-\beta_{i+1}})\bfx_{i+1} + \beta_{i+1} \bfs_\bftheta(\bfx_{i+1}, t_{i+1})$}}\vspace{0.35em}
                 \State{$\bfz \sim \mcal{N}(\bfzero, \bfI_d)$}
                 \State{$\bfx_i \gets \bfx_i' + \sqrt{\beta_{i+1}} \bfz$}
                 \For{$j=1$ {\bfseries to} $M$}
                    \State{$\bfz \sim \mcal{N}(\bfzero, \bfI_d)$}
                    \State{$\bfx_{i} \gets \bfx_{i} + \epsilon_i \bfs_\bftheta(\bfx_{i}, t_{i}) + \sqrt{2\epsilon_i}\bfz$}
                 \EndFor
               \EndFor
               \State {\bfseries return} $\bfx_0$
            \end{algorithmic}
    \end{algorithm}
\end{minipage}
\fi



When using the reverse diffusion sampling method as the predictor, and annealed Langevin MCMC as the corrector, we have Alg.~1 and Alg.~2 for NCSN and DDPM respectively, where $M$ represents the number of Langevin sampling steps per noise scale. In addition, we use $\{\delta_i\}_{i=0}^{N-1}$ and $\{\epsilon_i\}_{i=0}^{N-1}$ to denote step size schedules for Langevin dynamics. In our experiments, we take the schedule of annealed Langevin dynamics in \citet{song2019generative}, but modify it slightly in order to achieve better empirical performance (see Appendix for details). Algs.~1 and 2 generalize the original sampling methods of NCSN and DDPM: We can recover annealed Langevin dynamics for NCSN by removing the predictor part, or regain the reverse diffusion sampling method for DDPM by removing the corrector, which equals the original DDPM sampling method in the limit of small time steps.

\paragraph{Error analysis} The error of sampling with the reverse-time SDE comes from two sources: discretization of the SDE, and estimation of the true scores. We can use a finer discretization and/or a higher-order numerical solver to reduce the discretization error, but this might lead to larger estimation errors since using more discretization steps amounts to evaluating score-based models at more time steps. The estimation errors of the score-based model at multiple time steps can compound. This estimation error can be reduced by incorporating the corrector step, because if the sampler used for the corrector step is accurate (which can be controlled by tuning the step sizes and number of sampling steps of the MCMC), the final samples will only come from the score-based model for the smallest noise scale, and are asymptotically agnostic to the estimation errors of other scores. PC samplers have the benefit of avoiding the accumulation of estimation errors over time.

\paragraph{PC improves performance} We train an NCSN and a DDPM model using the architecture in \cite{ho2020denoising} on CIFAR-10. Results in \cref{tab:compare_samplers} confirm that the reverse diffusion sampling method outperforms the DDPM sampling method. In addition, no matter what type of predictor method is used, adding corrector always gives better performance at the cost of more computation. \todo{results with the same computation.}

\paragraph{Predictor vs. corrector} We conduct an empirical study to demonstrate that in many cases, it is beneficial 
to split computation between the predictor and the corrector, rather than allocating all computation to either the predictor (as done in DDPM) or the corrector (as done in NCSN). As an illustration, we train a score-based model on $256\times 256$ LSUN bedrooms with the SDE of NCSN, and report the results of different computation allocation in \cref{fig:computation}.
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/computation.pdf}
    \caption{Predictor-corrector sampling for LSUN bedrooms. The vertical axis corresponds to the total computation, and the horizontal axis represents the amount of computation allocated to the corrector. Samples are the best when computation is split between the predictor and corrector. \todo{change it to 4x4 grids on both bedrooms and church/celeba-hq. }}
    \label{fig:computation}
\end{figure}

\begin{table}
	\caption{The performance of various samplers applied to NCSN/DDPM models trained on CIFAR-10. Results are averaged over 5 different set of samples. \todo{make this a bar plot instead of a table?}}\label{tab:compare_samplers}
	\centering
	\begin{adjustbox}{max width=\textwidth}
		\begin{tabular}{cccc}
			\Xhline{3\arrayrulewidth} \bigstrut
			Predictor & Corrector & Model & FID \\
			\Xhline{1\arrayrulewidth}\bigstrut
			reverse diffusion	& Yes &	NCSN & $3.60 \pm 0.02$\\
            DDPM sampling & Yes	& NCSN	& $3.62 \pm 0.03$\\
            gradient flow &	Yes	& NCSN	& $3.51 \pm 0.04$\\
            reverse diffuion & No & NCSN & $4.79 \pm 0.07$\\
            gradient flow & No & NCSN & $15.41 \pm 0.15$\\
            DDPM sampling & No & NCSN &	$4.98 \pm 0.06$\\
            reverse diffusion &	Yes & DDPM & $3.18 \pm 0.01$\\
            gradient flow & Yes & DDPM & $3.06 \pm 0.03$\\
            DDPM sampling &	Yes	& DDPM & $3.21 \pm 0.02$\\
            reverse diffuion & No & DDPM & $3.21 \pm 0.02$\\
            gradient flow & No & DDPM & $3.59 \pm 0.04$\\
            DDPM sampling & No & DDPM & $3.24 \pm 0.02$\\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	\end{adjustbox}
\end{table}


\subsection{Probability flow sampling}
The score-based model enables another numerical method for solving the reverse-time SDE. %
For all diffusion processes, there exists a corresponding \emph{deterministic process} whose trajectories induce the same evolution of densities. This deterministic process satisfies an ODE given by deterministic particle flows, which can be derived from the SDE once scores are known. Therefore, we can produce data samples by integrating the associated ODE for the reverse-time SDE, and then collecting endpoints of the resulting trajectories. 

\begin{theorem}[Probability flows for SDEs]
Given the same $p_0(\bfx_0)$, particles flowing according to the following ODE share the same trajectories of densities as the SDE in \cref{eqn:forward_sde}:
\begin{align}
    \ud \bfx_t = \bigg\{\bff(\bfx_t, t) - \frac{1}{2} \nabla \cdot [\bfG(\bfx_t, t)\bfG(\bfx_t, t)\tran] - \frac{1}{2} \bfG(\bfx_t, t)\bfG(\bfx_t, t)\tran \nabla_\bfx \log p_t(\bfx_t)\bigg\} \ud t \label{eqn:flow}.
\end{align}
\end{theorem}

For sample generation, we can either solve the ODE with a fixed discretization strategy (named flow\textsubscript{d}) like the one in NCSN/DDPM, or a black-box integrator with adaptive step sizes and error control (named flow\textsubscript{c}) like in neural ODEs. Both sampling methods can generate reasonable samples with competitive FIDs, as demonstrated in \cref{tab:compare_samplers}. We can explicitly trade accuracy for efficiency with black-box solvers. With a larger error tolerance, the number of function evaluations for a black-box solver can be just $1/10$-th of other sampling methods. \todo{add experimental results here.}

\subsubsection{Exact likelihood computation}
Deterministic probability flows turn our time-dependent score-based model into a neural ODE~\citep{chen2018neural}. Leveraging this connection, we can compute the likelihood of our particle flow dynamics via the instantaneous change of variables formula:
\begin{theorem}[Likelihood of particle flows]
\begin{multline}
\log p_0(\bfx_0) = \log p_T(\bfx_T) + \\
\int \nabla \cdot \bff(\bfx_t, t) - \frac{1}{2} \nabla^2 \cdot [\bfG(\bfx_t, t)\bfG(\bfx_t, t)\tran] - \frac{1}{2} \nabla \cdot [\bfG(\bfx_t, t)\bfG(\bfx_t, t)\tran \nabla_\bfx \log p_t(\bfx_t)]  \ud t
\end{multline}\label{eqn:likelihood}
\end{theorem}
\begin{wraptable}[8]{l}{0.4\textwidth}
\vspace{-2em}
\centering
\caption{NLL on CIFAR-10}\label{tab:bpd}
\begin{adjustbox}{max width=0.4\textwidth}
    \begin{tabular}{l c}
    \toprule
    Model & NLL \\
    \midrule
    DDPM ($L_{\text{simple}}$) & $\leq 3.75$\\
    DDPM (ELBO) & $\leq 3.70$\\
    \midrule
    NCSN cont. & $3.66 \pm 0.0038$\\
    DDPM cont. & $3.40 \pm 0.0040$\\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\end{wraptable}
Here $\nabla^2 := \nabla \cdot \nabla$. The divergence $\nabla \cdot \bfa(\bfx)$ is oftentimes hard to compute, but has an unbiased estimator via Hutchinson's trace estimator~\citep{hutchinson1990stochastic}, \ie, $\nabla \cdot \bfa(\bfx) = \mbb{E}[\bfe \tran \nabla \bfa(\bfx) \bfe]$, where $\bfe$ is a Gaussian or Rademacher random variable, and $\nabla \bfa(\bfx)$ denotes the Jacobian of $\bfa(\bfx)$. Using \cref{eqn:likelihood} and Hutchinson's trace estimator, we can compute the exact likelihood on a test dataset with very small errors~\citep{grathwohl2019scalable}.

We report negative log-likelihoods (NLLs) measured in bits/dim in \cref{tab:bpd}. The likelihoods computed via particle flows are on uniform dequantized data. For DDPM, we obtain better bits/dim compared to the upper bound given by ELBO, since our likelihoods are exact.

\subsubsection{Latent representations}
By integrating \cref{eqn:flow}, we can encode any datapoint $\bfx_0$ into a latent space $\bfx_T$. Decoding can be achieved by integrating a corresponding ODE for the reverse-time SDE. Same as other invertible models such neural ODEs and normalizing flows~\citep{dinh2016density,song2019mintnet}, we can manipulate this latent representation for image editing, such as interpolation, and temperature scaling. \todo{Add experimental results}

There is one special difference from other invertible models: our representation is uniquely identifiable, meaning that with sufficient training data, model capacity, and optimization accuracy, the encoding for a same input always stays the same. This is because our forward SDE, \cref{eqn:forward_sde}, is prescribed without trainable parameters, and its associated particle flow ODE, \cref{eqn:flow}, provides the same trajectories given perfectly estimated scores. \todo{add a quick figure to verify this.}


\section{Controllable generation}
The continuous structure of our framework allows us to not only produce data samples from $p_0(\bfx_0)$, but also control this sampling process for a multitude of other tasks. Let $p_t(\bfx_t \mid \bfy)$ be the posterior distribution of $p_t(\bfx_t)$ given the additional information $\bfy$. We provide a principled method to sample from $p_0(\bfx_0 \mid \bfy)$ at test time for an unconditional score-based model, without re-training it on additional information. The method can be applied to image inpainting, colorization, class-conditional sample generation and others by training a single time-dependent score-based model.


\begin{theorem}[Conditional reverse-time SDE]
Trajectories of the reverse-time SDE
\begin{multline}
\ud \bfx_t = \{\bff(\bfx_t, t) - \nabla \cdot [\bfG(\bfx_t, t) \bfG(\bfx_t,t)\tran] - \bfG(\bfx_t,t)\bfG(\bfx_t,t)\tran  \nabla_\bfx  \log p_t(\bfx_t)\\ - \bfG(\bfx_t,t)\bfG(\bfx_t,t)\tran  \nabla_\bfx  \log p_t(\bfy \mid \bfx_t)\} \ud t + \mbf{G}(\bfx_t, t) \ud \bar{\bfw}_t
\end{multline}
satisfy the marginal probability $p_t(\bfx_t \mid \bfy)$ at time $t$.
\end{theorem}


\subsection{Class-conditional sampling}
When $\bfy$ represents class labels, we can train a time-dependent classifier $p_t(\bfy \mid \bfx_t)$ for class-conditional sampling. Since the forward SDE is tractable, we can easily create a pair of training data $(\bfx_t, \bfy)$ by first sampling $(\bfx_0, \bfy)$ from a dataset and then obtaining $\bfx_t \sim p_{0t}(\bfx_t \mid \bfx_0)$. Afterwards, we may employ a mixture of cross-entropy losses over different time steps, like \cref{eqn:training}, to train the time-dependent classifier $p_t(\bfy \mid \bfx_t)$.

\todo{add pictures}

\subsection{Imputation} 
Imputation is a special case of conditional sampling. Denote by $\Omega(\bfx)$ and $\bar{\Omega}(\bfx)$ the known and unknown dimensions of $\bfx$ respectively, and let $\bff_\Omega(\cdot, t)$ and $\bfG_\Omega(\cdot, t)$ denote $\bff(\cdot, t)$ and $\bfG(\cdot, t)$ restricted to the known dimensions. When $\bff(\cdot, t)$ is element-wise (true for NCSN/DDPM), $\bff_\Omega(\cdot, t)$ denotes the same element-wise function applied only to the known dimensions. When $\bfG(\cdot, t)$ is diagonal (true for NCSN/DDPM), $\bfG_\Omega(\cdot, t)$ is the sub-matrix of known dimensions. 

We aim to sample from $p(\bar{\Omega}(\bfx_0) \mid \Omega(\bfx_0) = \bfy)$. Let $\bfz_t = \Omega(\bfx_t)$. The SDE for $\bfz_t$ can be written as
\begin{align*}
\ud \bfz_t = \bff_\Omega(\bfz_t, t) dt + \bfG_\Omega(\bfz_t, t) \ud \bfw_t,
\end{align*}
The reverse diffusion, given $\Omega(\bfx_0) = \bfy$, is
\begin{align*}
\ud\bfz_t = (\bff_\Omega(\bfz_t, t) - \bfG_\Omega(\bfz_t, t)\bfG_\Omega(\bfz_t, t)\tran \nabla_\bfz \log p_t(\bfz_t \mid \Omega(\bfz_0) = \bfy))\ud t + \bfG_\Omega(\bfz_t, t)\ud\bar{\bfw}_t.
\end{align*}
Although $p_t(\bfz_t \mid \Omega(\bfx_0) = \bfy)$ is in general intractable, it can be approximated by
\begin{align*}
p_t(\bfz_t \mid \Omega(\bfx_0) = \bfy) &= \int p_t(\bfz_t \mid \Omega(\bfx_t), \bfy) p_t(\Omega(\bfx_t) \mid \bfy) \ud \Omega(\bfx_t) \\
&= \mathbb{E}_{p_t(\Omega(\bfx_t) \mid \bfy)}[p_t(\bfz_t \mid \Omega(\bfx_t), \bfy)]\\
&\approx \mathbb{E}_{p_t(\Omega(\bfx_t) \mid \bfy)}[p_t(\bfz_t \mid \Omega(\bfx_t))]\\
&\approx p_t(\bfz_t \mid \Omega'(\bfx_t)),
\end{align*}
where $\Omega'(\bfx_t) \sim p_t(\Omega(\bfx_t) \mid \bfy)$.
Therefore,
\begin{align*}
\nabla_\bfz \log p_t(\bfz_t \mid \Omega(\bfx_0)=\bfy) &\approx \nabla_\bfz \log p_t(\bfz_t \mid \Omega'(\bfx_t)) \\
&= \nabla_\bfz \log p_t([\bfz_t; \Omega'(\bfx_t)]).
\end{align*}

Colorization is a special case of imputation, except for the known data dimensions are coupled. We can decouple these data dimensions with an orthogonal linear transformation, and perform imputation in the transformed space. \todo{include proof-of-concept images.}

==> score sde (v2)_arXiv/sampling.tex <==
\section{Solving the reverse SDE}
After training a time-dependent score-based model $\bfs_\bftheta$, we can use it to construct the reverse-time SDE and then simulate it with numerical approaches to generate samples from $p_0$. %

\subsection{General-purpose numerical SDE solvers}

Numerical solvers provide approximate trajectories from SDEs. Many general-purpose numerical methods exist for solving SDEs, such as Euler-Maruyama and stochastic Runge-Kutta methods~\citep{kloeden2013numerical}, which correspond to different discretizations of the stochastic dynamics. We can apply any of them to the reverse-time SDE for sample generation. %

Ancestral sampling, the sampling method of DDPM (\cref{eqn:ddpm_sampling}), actually corresponds to one special discretization of the reverse-time VP SDE (\cref{eqn:ddpm_sde}) (see \cref{app:reverse_diffusion}). Deriving the ancestral sampling rules for new SDEs, however, can be non-trivial. To remedy this, we propose \emph{reverse diffusion samplers} (details in \cref{app:reverse_diffusion}), which discretize the reverse-time SDE in the same way as the forward one, and thus can be readily derived given the forward discretization.
As shown in \cref{tab:compare_samplers}, reverse diffusion samplers perform slightly better than ancestral sampling for both SMLD and DDPM models on CIFAR-10 (DDPM-type ancestral sampling is also applicable to SMLD models, see \cref{app:ancestral}.)


\subsection{Predictor-corrector samplers}
Unlike generic SDEs, we have additional information that can be used to improve solutions. Since we have a score-based model $\bfs_{\bftheta^*}(\bfx, t) \approx \nabla_\bfx \log p_t(\bfx)$, we can employ score-based MCMC approaches, such as Langevin MCMC~\citep{parisi1981correlation,grenander1994representations} or HMC~\citep{neal2011mcmc} to sample from $p_t$ directly, and correct the solution of a numerical SDE solver. 

Specifically, at each time step, the numerical SDE solver first gives an estimate of the sample at the next time step, playing the role of a ``predictor''. Then, the score-based MCMC approach corrects the 
marginal distribution of the estimated sample, playing the role of a ``corrector''. The idea is analogous to Predictor-Corrector methods, a family of numerical continuation techniques for solving systems of equations~\citep{allgower2012numerical}, and we similarly name our hybrid sampling algorithms \emph{Predictor-Corrector} (PC) samplers. Please find pseudo-code and a complete description in \cref{app:pc}. PC samplers generalize the original sampling methods of SMLD and DDPM: the former uses an identity function as the predictor and annealed Langevin dynamics as the corrector, while the latter uses ancestral sampling as the predictor and identity as the corrector. %

\begin{table}
    \definecolor{h}{gray}{0.9}
	\caption{Comparing different reverse-time SDE solvers on CIFAR-10. Shaded regions are obtained with the same computation (number of score function evaluations). Mean and standard deviation are reported over five sampling runs. ``P1000'' or ``P2000'': predictor-only samplers using 1000 or 2000 steps. ``C2000'': corrector-only samplers using 2000 steps. ``PC1000'': Predictor-Corrector (PC) samplers using 1000 predictor and 1000 corrector steps.}\label{tab:compare_samplers}
	\centering
	\begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{c|c|c|c|c|c|c|c|c}
			\Xhline{3\arrayrulewidth} \bigstrut
			  & \multicolumn{4}{c|}{Variance Exploding SDE (SMLD)} & \multicolumn{4}{c}{Variance Preserving SDE (DDPM)}\\
			 \Xhline{1\arrayrulewidth}\bigstrut
			\diagbox[height=1cm, width=3cm]{Predictor}{FID$\downarrow$}{Sampler} & P1000 & \cellcolor{h}P2000 & \cellcolor{h}C2000 & \cellcolor{h}PC1000 & P1000 & \cellcolor{h}P2000 & \cellcolor{h}C2000 & \cellcolor{h}PC1000  \\
			\Xhline{1\arrayrulewidth}\bigstrut
            ancestral sampling & 4.98\scalebox{0.7}{ $\pm$ .06}	& \cellcolor{h}4.88\scalebox{0.7}{ $\pm$ .06} &\cellcolor{h} & \cellcolor{h}\textbf{3.62\scalebox{0.7}{ $\pm$ .03}} & 3.24\scalebox{0.7}{ $\pm$ .02}	& \cellcolor{h}3.24\scalebox{0.7}{ $\pm$ .02} &\cellcolor{h} & \cellcolor{h}\textbf{3.21\scalebox{0.7}{ $\pm$ .02}}\\
        	reverse diffusion & 4.79\scalebox{0.7}{ $\pm$ .07} & \cellcolor{h}4.74\scalebox{0.7}{ $\pm$ .08} & \cellcolor{h} & \cellcolor{h}\textbf{3.60\scalebox{0.7}{ $\pm$ .02}} & 3.21\scalebox{0.7}{ $\pm$ .02} & \cellcolor{h}3.19\scalebox{0.7}{ $\pm$ .02} & \cellcolor{h} &\cellcolor{h}\textbf{3.18\scalebox{0.7}{ $\pm$ .01}}\\
            probability flow &	15.41\scalebox{0.7}{ $\pm$ .15} &\cellcolor{h}10.54\scalebox{0.7}{ $\pm$ .08}&\cellcolor{h} \multirow{-3}{*}{20.43\scalebox{0.7}{ $\pm$ .07}} & \cellcolor{h}\textbf{3.51\scalebox{0.7}{ $\pm$ .04}} & 3.59\scalebox{0.7}{ $\pm$ .04} & \cellcolor{h}3.23\scalebox{0.7}{ $\pm$ .03} & \cellcolor{h}\multirow{-3}{*}{19.06\scalebox{0.7}{ $\pm$ .06}} & \cellcolor{h}\textbf{3.06\scalebox{0.7}{ $\pm$ .03}}\\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	\end{adjustbox}
\end{table}



We test PC samplers on SMLD and DDPM models (see \cref{alg:pc_smld,alg:pc_ddpm} in \cref{app:pc}) trained with original discrete objectives given by \cref{eqn:ncsn_obj,eqn:ddpm_obj}. %
This exhibits the compatibility of PC samplers to score-based models trained with a fixed number of noise scales. We summarize the performance of different samplers in \cref{tab:compare_samplers}, where probability flow is a predictor to be discussed in \cref{sec:flow}. Detailed experimental settings and additional results are given in \cref{app:pc}. We observe that our reverse diffusion sampler always outperform ancestral sampling, and corrector-only methods (C2000) perform worse than other competitors (P2000, PC1000) with the same computation (In fact, we need way more corrector steps per noise scale, and thus more computation, to match the performance of other samplers.) For all predictors, adding one corrector step for each predictor step (PC1000) doubles computation but always improves sample quality (against P1000). Moreover, it is typically better than doubling the number of predictor steps without adding a corrector (P2000), where we have to interpolate between noise scales in an ad hoc manner (detailed in \cref{app:pc}) for SMLD/DDPM models. In \cref{fig:computation} (\cref{app:pc}), we additionally provide qualitative comparison for models trained with the continuous objective \cref{eqn:training} on $256\times 256$ LSUN images and the VE SDE, where PC samplers clearly surpass predictor-only samplers under comparable computation, when using a proper number of corrector steps.








\subsection{Probability flow and connection to neural ODEs}\label{sec:flow}
Score-based models enable another numerical method for solving the reverse-time SDE. For all diffusion processes, there exists a corresponding \emph{deterministic process} whose trajectories share the same marginal probability densities $\{p_t(\bfx)\}_{t=0}^T$ as the SDE. This deterministic process satisfies an ODE~(more details in \cref{app:prob_flow_derive}):
\begin{align}
    \ud \bfx = \Big[\bff(\bfx, t) - \frac{1}{2} g(t)^2\nabla_\bfx \log p_t(\bfx)\Big] \ud t, \label{eqn:flow}
\end{align}
which can be determined from the SDE once scores are known. We name the ODE in \cref{eqn:flow} the \emph{probability flow ODE}.
When the score function is approximated by the time-dependent score-based model, which is typically a neural network, this is an example of a neural ODE~\citep{chen2018neural}. 



\textbf{Exact likelihood computation}~ Leveraging the connection to neural ODEs, we can compute the density defined by \cref{eqn:flow}  via the instantaneous change of variables formula \citep{chen2018neural}. This allows us to compute the \emph{exact likelihood on any input data} (details in \cref{app:prob_flow_likelihood}). %
As an example, we report negative log-likelihoods (NLLs) measured in bits/dim on the CIFAR-10 dataset in \cref{tab:bpd}. We compute log-likelihoods on uniformly dequantized data, and only compare to models evaluated in the same way (omitting models evaluated with variational dequantization~\citep{ho2019flow++} or discrete data), except for DDPM ($L$/$L_\text{simple}$) whose ELBO values (annotated with *) are reported on discrete data. Main results: (i) For the same DDPM model in \citet{ho2020denoising}, we obtain better bits/dim than ELBO, since our likelihoods are exact; (ii) Using the same architecture, we trained another DDPM model with the continuous objective in \cref{eqn:training} (\ie, DDPM cont.), which further improves the likelihood; (iii) With sub-VP SDEs, we always get higher likelihoods compared to VP SDEs; (iv) With improved architecture (\ie, DDPM++ cont., details in \cref{sec:arch}) and the sub-VP SDE, we can set a new record bits/dim of 2.99 on uniformly dequantized CIFAR-10 even \emph{without maximum likelihood training}.

\begin{table}
\begin{minipage}[t]{0.48\textwidth}
\vspace{-0.3cm}
\begin{table}[H]
\centering
\caption{NLLs and FIDs (ODE) on CIFAR-10. }\label{tab:bpd}\vspace{-1em}
\footnotesize
 \setlength\tabcolsep{3.5pt}
\begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l c c}
    \toprule
    Model & NLL Test $\downarrow$ & FID $\downarrow$\\
    \midrule
    RealNVP~\citep{dinh2016density} & 3.49 & -\\
    iResNet~\citep{behrmann2019invertible} & 3.45 & -\\
    Glow~\citep{kingma2018glow} & 3.35 & - \\
    MintNet~\citep{song2019mintnet} & 3.32 & - \\
    Residual Flow~\citep{chen2019residual} & 3.28 & 46.37\\
    FFJORD~\citep{grathwohl2018ffjord} & 3.40 & -\\
    Flow++~\citep{ho2019flow++} & 3.29 & -\\
    DDPM ($L$)~\citep{ho2020denoising} & $\leq$ 3.70\textsuperscript{*} & 13.51\\
    DDPM ($L_{\text{simple}}$)~\citep{ho2020denoising} & $\leq$ 3.75\textsuperscript{*} & 3.17\\
    \midrule
    DDPM & 3.28 & 3.37\\\relax
    DDPM cont. (VP) & 3.21 & 3.69\\\relax
    DDPM cont. (sub-VP) & 3.05 & 3.56\\\relax
    DDPM++ cont. (VP) & 3.16 & 3.93\\\relax
    DDPM++ cont. (sub-VP) & 3.02 & 3.16\\ \relax
    DDPM++ cont. (deep, VP) & 3.13 & 3.08\\ \relax
    DDPM++ cont. (deep, sub-VP) & \textbf{2.99} & \textbf{2.92} \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\end{table}
\end{minipage}\hfil
\begin{minipage}[t]{0.48\textwidth}
\vspace{-0.3cm}
\begin{table}[H]
\centering
\caption{CIFAR-10 sample quality.}\label{tab:fid}\vspace{-1em}
\footnotesize
 \setlength\tabcolsep{3.5pt}
\begin{adjustbox}{max width=\textwidth}
  \begin{tabular}{lcc}
    \toprule
    Model & FID$\downarrow$ & IS$\uparrow$  \\
        \midrule
      {\bf Conditional} & & \\
      \midrule
      BigGAN~\citep{brock2018large} & 14.73 & 9.22 \\
      StyleGAN2-ADA~\citep{karras2020training} & \textbf{2.42} & \textbf{10.14} \\
      \midrule
      {\bf Unconditional} & & \\
      \midrule
      StyleGAN2-ADA~\citep{karras2020training} & 2.92 & 9.83 \\
      NCSN~\citep{song2019generative} & 25.32 & 8.87 $\pm$ .12 \\
      NCSNv2~\citep{song2020improved} & 10.87 & 8.40 $\pm$ .07\\
      DDPM~\citep{ho2020denoising} & 3.17 & 9.46 $\pm$ .11\\
      \midrule
      DDPM++ & 2.78 & 9.64\\
      DDPM++ cont. (VP) & 2.55 & 9.58 \\
      DDPM++ cont. (sub-VP) & 2.61 & 9.56 \\
      DDPM++ cont. (deep, VP) & 2.41 & 9.68\\
      DDPM++ cont. (deep, sub-VP) & 2.41 & 9.57\\
      NCSN++ & 2.45 & 9.73 \\
      NCSN++ cont. (VE) & 2.38 & 9.83\\
      NCSN++ cont. (deep, VE) & \textbf{2.20} & \textbf{9.89}\\
    \bottomrule 
    \end{tabular}
\end{adjustbox}
\end{table}
\end{minipage}
\end{table}

\textbf{Manipulating latent representations}~ By integrating \cref{eqn:flow}, we can encode any datapoint $\bfx(0)$ into a latent space $\bfx(T)$. Decoding can be achieved by integrating a corresponding ODE for the reverse-time SDE. As is done with other invertible models such as neural ODEs and normalizing flows~\citep{dinh2016density,kingma2018glow}, we can manipulate this latent representation for image editing, such as interpolation, and temperature scaling (see \cref{fig:prob_flow} and \cref{app:flow}). 

\textbf{Uniquely identifiable encoding}~ Unlike most current invertible models, 
our encoding is {\em uniquely identifiable}, meaning that with sufficient training data, model capacity, and optimization accuracy, the encoding for an input is uniquely determined by the data distribution \citep{roeder2020linear}. This is because our forward SDE, \cref{eqn:forward_sde}, has no trainable parameters, and its associated probability flow ODE, \cref{eqn:flow}, provides the same trajectories given perfectly estimated scores. We provide additional empirical verification on this property in \cref{app:identifiability}.

\textbf{Efficient sampling}~ As with neural ODEs, we can sample $\bfx(0) \sim p_0$ by solving \cref{eqn:flow} from different final conditions $\bfx(T)\sim p_T$. Using a fixed discretization strategy we can generate competitive samples, especially when used in conjuction with correctors (\cref{tab:compare_samplers},  ``probability flow sampler'', details in \cref{app:prob_flow_sampling}). Using a black-box ODE solver~\citep{dormand1980family} not only produces high quality samples (\cref{tab:bpd}, details in \cref{app:flow}), but also allows us to explicitly trade-off accuracy for efficiency. With a larger error tolerance, the number of function evaluations can be reduced by over $90\%$ without affecting the visual quality of samples (\cref{fig:prob_flow}).
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/ode_tight}
    \vspace{-5mm}
    \caption{{\bf Probability flow ODE enables fast sampling} with adaptive stepsizes as the numerical precision is varied (\textit{left}), and reduces the number of score function evaluations (NFE) without harming quality (\textit{middle}). The invertible mapping from latents to images allows for interpolations (\textit{right}).}
    \label{fig:prob_flow}
\end{figure}



\subsection{Architecture improvements}\label{sec:arch}



We explore several new architecture designs for score-based models using both VE and VP SDEs (details in \cref{app:arch_search}), where we train models with the same discrete objectives as in SMLD/DDPM. We directly transfer the architectures for VP SDEs to sub-VP SDEs due to their similarity. Our optimal architecture for the VE SDE, named NCSN++, achieves an FID of 2.45 on CIFAR-10 with PC samplers, while our optimal architecture for the VP SDE, called DDPM++, achieves 2.78.

By switching to the continuous training objective in \cref{eqn:training}, and increasing the network depth, we can further improve sample quality for all models. The resulting architectures are denoted as NCSN++ cont. and DDPM++ cont. in \cref{tab:fid} for VE and VP/sub-VP SDEs respectively. Results reported in \cref{tab:fid} are for the checkpoint with the smallest FID over the course of training, where samples are generated with PC samplers. In contrast, FID scores and NLL values in \cref{tab:bpd} are reported for the last training checkpoint, and samples are obtained with black-box ODE solvers. As shown in \cref{tab:fid}, VE SDEs typically provide better sample quality than VP/sub-VP SDEs, but we also empirically observe that their likelihoods are worse than VP/sub-VP SDE counterparts. This indicates that practitioners likely need to experiment with different SDEs for varying domains and architectures.

Our best model for sample quality, NCSN++ cont. (deep, VE), doubles the network depth and sets new records for both inception score and FID on unconditional generation for CIFAR-10. Surprisingly, we can achieve better FID than the previous best conditional generative model without requiring labeled data. With all improvements together, we also obtain the first set of high-fidelity samples on CelebA-HQ $1024\times 1024$ from score-based models (see \cref{app:hq}). Our best model for likelihoods, DDPM++ cont. (deep, sub-VP), similarly doubles the network depth and achieves a log-likelihood of 2.99 bits/dim with the continuous objective in \cref{eqn:training}. To our best knowledge, this is the highest likelihood on uniformly dequantized CIFAR-10.



==> score sde (v2)_arXiv/sdes_new.tex <==
\section{Score-based generative modeling with SDEs}
Perturbing data with multiple noise scales is key to the success of previous methods. We propose to generalize this idea further to an infinite number of noise scales, such that perturbed data distributions evolve according to an SDE as the noise intensifies. %
An overview of our framework is given in \cref{fig:toy}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth, trim=16 0 12 14, clip]{figures/teaser.pdf}
    \caption{\textbf{Overview of score-based generative modeling through SDEs}. We can map data to a noise distribution (the prior) with an SDE (\cref{sec:sde_perturb}), and reverse this SDE for generative modeling (\cref{sec:sde_reverse}). We can also reverse the associated probability flow ODE (\cref{sec:flow}), which yields a deterministic process that samples from the same distribution as the SDE. Both the reverse-time SDE and probability flow ODE can be obtained by estimating the score $\nabla_\bfx \log p_t(\bfx)$ (\cref{sec:training}).}
    \label{fig:toy}
\end{figure}

\subsection{Perturbing data with SDEs}\label{sec:sde_perturb}
Our goal is to construct a diffusion process $\{\bfx(t)\}_{t=0}^T$ indexed by a continuous time variable $t\in [0,T]$, such that $\bfx(0) \sim p_{0}$, for which we have a dataset of \iid samples, and $\bfx(T) \sim p_T$, for which we have a tractable form to generate samples efficiently. In other words, $p_0$ is the data distribution and $p_T$ is the prior distribution. This diffusion process can be modeled as the solution to an It\^{o} SDE:
\begin{align}
    \ud \bfx = \bff(\bfx, t) \ud t + {g}(t) \ud \bfw, \label{eqn:forward_sde}
\end{align}
where $\bfw$ is the standard Wiener process (\aka, Brownian motion), $\bff(\cdot, t): \mbb{R}^d \to \mbb{R}^d$ is a vector-valued function called the \emph{drift} coefficient of $\bfx(t)$, and ${g}(\cdot): \mbb{R} \to \mbb{R}$ is a scalar function known as the \emph{diffusion} coefficient of $\bfx(t)$. For ease of presentation we assume the diffusion coefficient is a scalar (instead of a $d \times d$ matrix) and does not depend on $\bfx$, but our theory can be generalized to hold in those cases (see \cref{app:general_sde}). The SDE has a unique strong solution as long as the coefficients are globally Lipschitz in both state and time~\citep{oksendal2003stochastic}. %
We hereafter denote by $p_t(\bfx)$ the probability density of $\bfx(t)$, and use $p_{st}(\bfx(t) \mid \bfx(s))$ to denote the transition kernel from $\bfx(s)$ to $\bfx(t)$, where $0 \leq s < t \leq T$.

Typically, $p_T$ is an unstructured prior distribution that contains no information of $p_0$, such as a Gaussian distribution with fixed mean and variance. There are various ways of designing the SDE in \cref{eqn:forward_sde} such that it diffuses the data distribution into a fixed prior distribution. We provide several examples later in \cref{sec:sde_examples} that are derived from continuous generalizations of SMLD and DDPM.

\subsection{Generating samples by reversing the SDE}\label{sec:sde_reverse}
By starting from samples of $\bfx(T) \sim p_T$ and reversing the process, we can obtain samples $\bfx(0)\sim p_0$. %
A remarkable result from~\citet{Anderson1982-ny} states that the reverse of a diffusion process is also a diffusion process, running backwards in time and given by the reverse-time SDE:
\begin{align}
    \ud \bfx = [\bff(\bfx, t) - g(t)^2  \nabla_{\bfx}  \log p_t(\bfx)] \ud t + g(t) \ud \bar{\bfw},\label{eqn:backward_sde}
\end{align}
where $\bar{\bfw}$ is a standard Wiener process
when time flows backwards from $T$ to $0$, and $\ud t$ is an infinitesimal negative timestep. Once the score of each marginal distribution, $\nabla_\bfx \log p_t(\bfx)$, is known for all $t$, we can derive the reverse diffusion process from \cref{eqn:backward_sde} and simulate it to sample from $p_0$.


\subsection{Estimating scores for the SDE}\label{sec:training}
The score of a distribution can be estimated by training a score-based model on samples with score matching~\citep{hyvarinen2005estimation,song2019sliced}. To estimate $\nabla_\bfx \log p_t(\bfx)$, we can train a time-dependent score-based model $\bfs_\bftheta(\bfx, t)$ via a continuous generalization to \cref{eqn:ncsn_obj,eqn:ddpm_obj}:
\begin{align}
   \bftheta^* = \argmin_\bftheta 
   \mbb{E}_{t}\Big\{\lambda(t) \mbb{E}_{\bfx(0)}\mbb{E}_{\bfx(t) \mid \bfx(0) }
   \big[\norm{\bfs_\bftheta(\bfx(t), t) - \nabla_{\bfx(t)}\log p_{0t}(\bfx(t) \mid \bfx(0))}_2^2 \big]\Big\}%
   . \label{eqn:training}
\end{align}
Here $\lambda: [0, T] \to \mbb{R}_{>0}$ is a positive weighting function, $t$ is uniformly sampled over $[0, T]$, $\bfx(0) \sim p_0(\bfx)$ and $\bfx(t) \sim p_{0t}(\bfx(t) \mid \bfx(0))$. With sufficient data and model capacity, score matching ensures that the optimal solution to \cref{eqn:training}, denoted by $\bfs_{\bftheta^\ast}(\bfx, t)$, equals $\nabla_\bfx \log p_t(\bfx)$ for almost all $\bfx$ and $t$. As in SMLD and DDPM, we can typically choose $\lambda \propto 1/{\mbb{E}\big[\norm{\nabla_{\bfx(t)}\log p_{0t}(\bfx(t) \mid \bfx(0))}_2^2\big]}$. Note that \cref{eqn:training} uses denoising score matching, but other score matching objectives, such as sliced score matching~\citep{song2019sliced} and finite-difference score matching~\citep{pang2020efficient} are also applicable here. 

We typically need to know the transition kernel $p_{0t}(\bfx(t) \mid \bfx(0))$ to efficiently solve \cref{eqn:training}. When $\bff(\cdot, t)$ is affine, the transition kernel is always a Gaussian distribution, where the mean and variance are often known in closed-forms and can be obtained with standard techniques (see Section 5.5 in \citet{sarkka2019applied}). For more general SDEs, we may solve Kolmogorov's forward equation~\citep{oksendal2003stochastic} to obtain $p_{0t}(\bfx(t) \mid \bfx(0))$. Alternatively, we can simulate the SDE to sample from $p_{0t}(\bfx(t) \mid \bfx(0))$ and replace denoising score matching in \cref{eqn:training} with sliced score matching for model training, which bypasses the computation of $\nabla_{\bfx(t)} \log p_{0t}(\bfx(t) \mid \bfx(0))$ (see \cref{app:general_sde}).




\subsection{Examples: VE, VP SDEs and beyond}\label{sec:sde_examples}
The noise perturbations used in SMLD and DDPM can be regarded as discretizations of two different SDEs. %
Below we provide a brief discussion and relegate more details to \cref{app:sde_derive}.

When using a total of $N$ noise scales, each perturbation kernel $p_{\sigma_i}(\bfx \mid \bfx_0)$ of SMLD corresponds to the distribution of $\bfx_i$ in the following Markov chain:
\begin{align}
\bfx_i = \bfx_{i-1} + \sqrt{\sigma_{i}^2 - \sigma_{i-1}^2} \bfz_{i-1}, \quad i=1,\cdots,N \label{eqn:ncsn},
\end{align}
where $\bfz_{i-1} \sim \mcal{N}(\bfzero, \bfI)$, and we have introduced $\sigma_0 = 0$ to simplify the notation.
In the limit of $N \to \infty$, $\{\sigma_i\}_{i=1}^N$ becomes a function $\sigma(t)$, $\bfz_i$ becomes $\bfz(t)$, and the Markov chain $\{\bfx_i\}_{i=1}^N$ becomes a continuous stochastic process $\{\bfx(t)\}_{t=0}^1$, where we have used a continuous time variable $t \in [0, 1]$ for indexing, rather than an integer $i$. The process $\{\bfx(t)\}_{t=0}^1$ is given by the following SDE
\begin{align}
\ud \bfx = \sqrt{\frac{\ud \left[ \sigma^2(t) \right]}{\ud t}}\ud \bfw. \label{eqn:ncsn_sde}
\end{align}
Likewise for the perturbation kernels $\{p_{\alpha_i}(\bfx \mid \bfx_0)\}_{i=1}^N$ of DDPM, the discrete Markov chain is
\begin{align}
    \bfx_i = \sqrt{1-\beta_{i}} \bfx_{i-1} + \sqrt{\beta_{i}} \bfz_{i-1}, \quad i=1,\cdots,N. \label{eqn:ddpm}
\end{align}
As $N\to \infty$, \cref{eqn:ddpm} converges to the following SDE,
\begin{align}
\ud \bfx = -\frac{1}{2}\beta(t) \bfx~ \ud t + \sqrt{\beta(t)} ~\ud \bfw. \label{eqn:ddpm_sde}
\end{align}

Therefore, the noise perturbations used in SMLD and DDPM correspond to discretizations of SDEs \cref{eqn:ncsn_sde,eqn:ddpm_sde}. Interestingly, the SDE of \cref{eqn:ncsn_sde} always gives a process with exploding variance when $t \to \infty$, whilst the SDE of \cref{eqn:ddpm_sde} yields a process with a fixed variance of one when the initial distribution has unit variance (proof in \cref{app:sde_derive}). Due to this difference, we hereafter refer to \cref{eqn:ncsn_sde} as the Variance Exploding (VE) SDE, and \cref{eqn:ddpm_sde} the Variance Preserving (VP) SDE. 

Inspired by the VP SDE, we propose a new type of SDEs which perform particularly well on likelihoods (see \cref{sec:flow}), given by
\begin{align}
    \ud \bfx = -\frac{1}{2}\beta(t) \bfx~ \ud t + \sqrt{\beta(t)(1 - e^{-2\int_0^t \beta(s)\ud s})} \ud \bfw.\label{eqn:subvp_sde}
\end{align}
When using the same $\beta(t)$ and starting from the same initial distribution, the variance of the stochastic process induced by \cref{eqn:subvp_sde} is always bounded by the VP SDE at every intermediate time step (proof in \cref{app:sde_derive}). For this reason, we name \cref{eqn:subvp_sde} the sub-VP SDE.

Since VE, VP and sub-VP SDEs all have affine drift coefficients, their perturbation kernels $p_{0t}(\bfx(t) \mid \bfx(0))$ are all Gaussian and can be computed in closed-forms, as discussed in \cref{sec:training}. This makes training with \cref{eqn:training} particularly efficient. 








